AI, Meet Human: Learning Paradigms for Hybrid Decision Making Systems

Everyday we increasingly rely on machine learning models to automate and support high-stake tasks and decisions. This growing presence means that humans are now constantly interacting with machine learning-based systems, training and using models everyday. Several different techniques in computer science literature account for the human interaction with machine learning systems, but their classification is sparse and the goals varied. This survey proposes a taxonomy of Hybrid Decision Making Systems, providing both a conceptual and technical framework for understanding how current computer science literature models interaction between humans and machines.

==> out <==
This is pdfTeX, Version 3.141592653-2.6-1.40.25 (TeX Live 2023/Arch Linux) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2022-11-01> patch level 1
L3 programming layer <2023-02-22> (./acmart.cls
Document Class: acmart 2022/10/24 v1.88 Typesetting articles for the Associatio
n for Computing Machinery
(/usr/share/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/share/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/share/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/share/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/share/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/share/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/share/texmf-dist/tex/latex/amscls/amsart.cls
Document Class: amsart 2020/05/29 v2.20.6
(/usr/share/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/share/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/share/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/share/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/share/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texmf-dist/tex/latex/refcount/refcount.sty
(/usr/share/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/share/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/share/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/share/texmf-dist/tex/latex/everyshi/everyshi.sty))
(/usr/share/texmf-dist/tex/latex/environ/environ.sty
(/usr/share/texmf-dist/tex/latex/trimspaces/trimspaces.sty))
(/usr/share/texmf-dist/tex/latex/textcase/textcase.sty)
(/usr/share/texmf-dist/tex/latex/hyperxmp/hyperxmp.sty
(/usr/share/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/share/texmf-dist/tex/latex/kvsetkeys/kvsetkeys.sty))
(/usr/share/texmf-dist/tex/generic/pdfescape/pdfescape.sty
(/usr/share/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty))
(/usr/share/texmf-dist/tex/generic/stringenc/stringenc.sty)
(/usr/share/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/share/texmf-dist/tex/latex/ifmtarg/ifmtarg.sty)
(/usr/share/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/ifdraft.sty)
(/usr/share/texmf-dist/tex/generic/iftex/ifluatex.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/share/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/share/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/share/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/share/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texmf-dist/tex/generic/gettitlestring/gettitlestring.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/share/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/share/texmf-dist/tex/latex/url/url.sty)
(/usr/share/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/share/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/share/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/share/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty
(/usr/share/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty)))
(/usr/share/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/share/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/share/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/share/texmf-dist/tex/latex/graphics/mathcolor.ltx))
(/usr/share/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/share/texmf-dist/tex/generic/iftex/ifvtex.sty))
(/usr/share/texmf-dist/tex/latex/ncctools/manyfoot.sty
(/usr/share/texmf-dist/tex/latex/ncctools/nccfoots.sty))
(/usr/share/texmf-dist/tex/generic/pdftex/glyphtounicode.tex)
(/usr/share/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/share/texmf-dist/tex/latex/base/fontenc.sty<<t1.cmap>>)
(/usr/share/texmf-dist/tex/latex/libertine/libertine.sty
(/usr/share/texmf-dist/tex/generic/iftex/ifxetex.sty)
(/usr/share/texmf-dist/tex/latex/base/textcomp.sty)
(/usr/share/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/share/texmf-dist/tex/latex/fontaxes/fontaxes.sty)
(/usr/share/texmf-dist/tex/latex/libertine/LinLibertine_I.tex))
(/usr/share/texmf-dist/tex/latex/inconsolata/zi4.sty
`inconsolata-zi4' v1.12, 2019/05/17 Text macros for Inconsolata (msharpe))
(/usr/share/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.71, 2022/01/16 Math macros based originally on txfonts (msharpe)
(/usr/share/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/share/texmf-dist/tex/generic/kastrup/binhex.tex)
amsthm NOT loaded
) (/usr/share/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texmf-dist/tex/latex/caption/caption3.sty
(/usr/share/texmf-dist/tex/latex/caption/caption-ams-smf.sto)))
(/usr/share/texmf-dist/tex/latex/float/float.sty)
(/usr/share/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment') Excluding comment 'CCSXML'
(/usr/share/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty) Special comment 'acks'
(/usr/share/texmf-dist/tex/latex/libertine/T1LinuxLibertineT-TLF.fd))
(/usr/share/texmf-dist/tex/latex/xargs/xargs.sty)
(/usr/share/texmf-dist/tex/latex/bbm-macros/bbm.sty)
(/usr/share/texmf-dist/tex/latex/optidef/optidef.sty
(/usr/share/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/share/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/share/texmf-dist/tex/latex/xifthen/xifthen.sty)
(/usr/share/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/share/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/share/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def))))
(/usr/share/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/share/texmf-dist/tex/latex/graphics/lscape.sty)
(/usr/share/texmf-dist/tex/latex/tools/longtable.sty)
(/usr/share/texmf-dist/tex/latex/todonotes/todonotes.sty
(/usr/share/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/share/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/share/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.tex)
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def)
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/share/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/share/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfkeyslibraryfiltered.code.te
x)) (/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.def
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-pdf.def)))
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigonometric.code
.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.random.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.comparison.code.te
x) (/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integerarithmetics
.code.tex) (/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfint.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconstruct.code.tex
) (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicstate.code.tex)

(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransformations.code.t
ex) (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathprocessing.code.te
x) (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransparency.code.tex)
 (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.tex)))
(/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.tex)
(/usr/share/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-0-65.sty)
(/usr/share/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-1-18.sty))
(/usr/share/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/share/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex))
(/usr/share/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothandlers.code.te
x) (/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
topaths.code.tex)))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
positioning.code.tex)) (/usr/share/texmf-dist/tex/latex/doublestroke/dsfont.sty
) (/usr/share/texmf-dist/tex/latex/makecell/makecell.sty
(/usr/share/texmf-dist/tex/latex/tools/array.sty))
(/usr/share/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/share/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
arrows.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/pgflibraryarrows.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.geometric.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.geomet
ric.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.misc.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.misc.c
ode.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.symbols.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.symbol
s.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.arrows.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.arrows
.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.callouts.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.callou
ts.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.multipart.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.multip
art.code.tex)))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
calc.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
decorations.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmoduledecorations.code.tex))
(/usr/share/texmf-dist/tex/latex/varwidth/varwidth.sty)
(/usr/share/texmf-dist/tex/latex/biblatex/biblatex.sty
(/usr/share/texmf-dist/tex/latex/logreq/logreq.sty
(/usr/share/texmf-dist/tex/latex/logreq/logreq.def))
(/usr/share/texmf-dist/tex/latex/biblatex/blx-dm.def)
(/usr/share/texmf-dist/tex/latex/biblatex/blx-compat.def)
(/usr/share/texmf-dist/tex/latex/biblatex/biblatex.def)
(/usr/share/texmf-dist/tex/latex/biblatex/blx-natbib.def) (./acmnumeric.bbx
(/usr/share/texmf-dist/tex/latex/biblatex-trad/trad-plain.bbx
(/usr/share/texmf-dist/tex/latex/biblatex-trad/trad-standard.bbx
(/usr/share/texmf-dist/tex/latex/biblatex/bbx/standard.bbx)))
(/usr/share/texmf-dist/tex/latex/biblatex-software/software.bbx
(/usr/share/texmf-dist/tex/latex/xurl/xurl.sty
xurl: Set penalties for biblatex
))) (./acmnumeric.cbx (/usr/share/texmf-dist/tex/latex/biblatex/cbx/numeric.cbx
)) (/usr/share/texmf-dist/tex/latex/biblatex/biblatex.cfg)
(/usr/share/texmf-dist/tex/latex/biblatex/blx-case-expl3.sty))
Excluding comment 'screenonly' Include comment 'printonly'
Include comment 'anonsuppress'

LaTeX Warning: Unused global option(s):
    [natbib=false].

(./main.aux (./appendices.aux))
(/usr/share/texmf-dist/tex/latex/newtx/omlnxlmi.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/share/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/share/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
(/usr/share/texmf-dist/tex/latex/libertine/OT1LinuxLibertineT-TLF.fd)<<ot1.cmap
>><<oml.cmap>> (/usr/share/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxsyc.fd) (./main.out) (./main.out)
(/usr/share/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/share/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/share/texmf-dist/tex/latex/upquote/upquote.sty)
(/usr/share/texmf-dist/tex/latex/caption/ltcaption.sty)

Package todonotes Warning: The length marginparwidth is less than 2cm and will 
most likely cause issues with the appearance of inserted todonotes. The issue c
an be solved by adding a line like \setlength {\marginparwidth }{2cm} prior to 
loading the todonotes package. on input line 144.

(/usr/share/texmf-dist/tex/latex/biblatex/lbx/american.lbx
(/usr/share/texmf-dist/tex/latex/biblatex-software/english-software.lbx
(/usr/share/texmf-dist/tex/latex/biblatex/lbx/english.lbx))
(/usr/share/texmf-dist/tex/latex/biblatex-software/english-software.lbx
(/usr/share/texmf-dist/tex/latex/biblatex/lbx/english.lbx))) (./main.bbl)
Excluding 'CCSXML' comment.
(/usr/share/texmf-dist/tex/latex/libertine/T1LinuxBiolinumT-TLF.fd)
(/usr/share/texmf-dist/tex/latex/libertine/TS1LinuxLibertineT-TLF.fd)
(/usr/share/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/share/texmf-dist/tex/latex/microtype/mt-msb.cfg) (./introduction.tex

LaTeX Warning: Citation 'dietvorst2015algorithm' on page 1 undefined on input l
ine 16.


LaTeX Warning: Citation 'lee2004trust' on page 1 undefined on input line 16.


LaTeX Warning: Citation 'dietvorst2015algorithm' on page 1 undefined on input l
ine 18.


LaTeX Warning: Citation 'logg2019algorithm' on page 1 undefined on input line 1
8.


Overfull \hbox (2.52794pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) assisted 

Overfull \hbox (5.77692pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Decision- 

Overfull \hbox (1.92734pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) making 

Overfull \hbox (3.57817pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Bucinca, 

Overfull \hbox (3.45026pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) man+AI 

Overfull \hbox (1.0689pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dently"[]  

Overfull \hbox (2.52794pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) assisted 

Overfull \hbox (5.77692pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Decision- 

Overfull \hbox (1.92734pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) making 

Overfull \hbox (3.57817pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Bucinca, 

Overfull \hbox (3.45026pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) man+AI 

Overfull \hbox (1.0689pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dently"[]  

LaTeX Warning: Citation 'rajpurkar2022ai' on page 1 undefined on input line 23.



LaTeX Warning: Citation 'goodell2021artificial' on page 1 undefined on input li
ne 23.


LaTeX Warning: Citation 'surden2019artificial' on page 1 undefined on input lin
e 23.


LaTeX Warning: Citation 'DBLP:conf/iclr/Saparov023' on page 1 undefined on inpu
t line 28.


LaTeX Warning: Citation 'DBLP:journals/tkdd/KaufmanRPS12' on page 1 undefined o
n input line 28.


LaTeX Warning: Citation 'DBLP:conf/nips/SolaimanD21' on page 1 undefined on inp
ut line 28.

[1.1{/var/lib/texmf/fonts/map/pdftex/updmap/pdftex.map}{/usr/share/texmf-dist/f
onts/enc/dvips/libertine/lbtn_25tcsq.enc}{/usr/share/texmf-dist/fonts/enc/dvips
/libertine/lbtn_76gpa5.enc}{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbt
n_naooyc.enc}{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_nh77jq.enc}{
/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_7grukw.enc}]

LaTeX Warning: Citation 'DBLP:conf/emnlp/CiosiciCLHFW21' on page 2 undefined on
 input line 51.


LaTeX Warning: Citation 'DBLP:conf/acl/ChenSFC0X23' on page 2 undefined on inpu
t line 51.


LaTeX Warning: Citation 'ferguson2020high' on page 2 undefined on input line 51
.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-1808-09123' on page 2 undefined
 on input line 53.


LaTeX Warning: Citation 'kempt2022m' on page 2 undefined on input line 53.


LaTeX Warning: Citation 'DBLP:conf/ijcai/RossHD17' on page 2 undefined on input
 line 53.


LaTeX Warning: Citation 'hildebrandt2013privacy' on page 2 undefined on input l
ine 56.


LaTeX Warning: Citation 'DBLP:conf/aaai/BansalW18' on page 2 undefined on input
 line 71.


LaTeX Warning: Citation 'DBLP:conf/hcomp/BansalNKLWH19' on page 2 undefined on 
input line 81.


Overfull \hbox (9.47112pt too wide) in paragraph at lines 81--81
\T1/LinuxLibertineT-TLF/m/n/6 (-20) bern[]etik[]es, 

Overfull \hbox (9.47112pt too wide) in paragraph at lines 81--81
\T1/LinuxLibertineT-TLF/m/n/6 (-20) bern[]etik[]es, 

LaTeX Warning: Citation 'dietvorst2018overcoming' on page 2 undefined on input 
line 81.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 2 undefined on input l
ine 82.

[2.2]

LaTeX Warning: Citation 'DBLP:journals/csur/YuZLHWJJ22' on page 3 undefined on 
input line 114.


LaTeX Warning: Citation '10.5555/3312046' on page 3 undefined on input line 114
.


LaTeX Warning: Citation 'DBLP:conf/ijcai/NobaniMM21' on page 3 undefined on inp
ut line 114.


Overfull \hbox (4.55762pt too wide) in paragraph at lines 168--169
 [][] 

Class acmart Warning: A possible image without description on input line 177.

[3.3]) (./paradigms.tex

Package caption Warning: \label without proper reference on input line 5.
See the caption package documentation for explanation.


LaTeX Warning: Reference `tbl:symbols' on page 4 undefined on input line 81.


LaTeX Warning: Citation 'Neykov2016' on page 4 undefined on input line 111.


LaTeX Warning: Citation 'Goodfellow2016' on page 4 undefined on input line 113.



LaTeX Warning: Citation 'Bartlett2006' on page 4 undefined on input line 113.


LaTeX Warning: Citation 'Lin2004' on page 4 undefined on input line 113.

[4.4{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_ki75ao.enc}{/usr/shar
e/texmf-dist/fonts/enc/dvips/libertine/lbtn_oexx6f.enc}] [5.5]

LaTeX Warning: Citation 'Lampert2016' on page 6 undefined on input line 130.


LaTeX Warning: Citation 'Kerrigan2021' on page 6 undefined on input line 132.

) (./human_oversight.tex

LaTeX Warning: Citation 'koulu2020proceduralizing' on page 6 undefined on input
 line 3.


LaTeX Warning: Citation 'quinonero2008dataset' on page 6 undefined on input lin
e 48.


Overfull \hbox (40.22641pt too wide) in paragraph at lines 48--54
[]\T1/LinuxLibertineT-TLF/m/it/10 (-20) Data shift. \T1/LinuxLibertineT-TLF/m/n
/10 (-20) Data shift is gen-er-ally in-tended as a change in the data dis-tri-b
u-tion [[]],
[6.6]

LaTeX Warning: Citation 'DBLP:journals/pacmhci/BucincaMG21' on page 7 undefined
 on input line 64.


LaTeX Warning: Citation 'parikh1994intuition' on page 7 undefined on input line
 67.


LaTeX Warning: Citation 'babuta2021machine' on page 7 undefined on input line 7
9.


LaTeX Warning: Citation 'malgieri2017right' on page 7 undefined on input line 7
9.


LaTeX Warning: Citation 'babuta2021machine' on page 7 undefined on input line 8
3.


LaTeX Warning: Citation 'ferguson2020high' on page 7 undefined on input line 83
.


LaTeX Warning: Citation 'gillespie2018custodians' on page 7 undefined on input 
line 83.


LaTeX Warning: Citation 'DBLP:conf/fat/RaghavanBKL20' on page 7 undefined on in
put line 84.


LaTeX Warning: Citation 'nahmias2021oversight' on page 7 undefined on input lin
e 87.


LaTeX Warning: Citation 'dietvorst2015algorithm' on page 7 undefined on input l
ine 108.


LaTeX Warning: Citation 'logg2019algorithm' on page 7 undefined on input line 1
08.


LaTeX Warning: Citation 'dietvorst2015algorithm' on page 7 undefined on input l
ine 110.


LaTeX Warning: Citation 'main2016cook' on page 7 undefined on input line 110.


Underfull \vbox (badness 1122) has occurred while \output is active [7.7]

LaTeX Warning: Citation 'alon2023human' on page 8 undefined on input line 124.


LaTeX Warning: Citation 'DBLP:journals/automatica/Bainbridge83' on page 8 undef
ined on input line 124.


LaTeX Warning: Citation 'ferguson2020high' on page 8 undefined on input line 12
4.


LaTeX Warning: Citation 'DBLP:conf/eaamo/Grgic-HlacaLWR22' on page 8 undefined 
on input line 125.


LaTeX Warning: Citation 'lee2018understanding' on page 8 undefined on input lin
e 125.


LaTeX Warning: Citation 'DBLP:conf/chi/0002HZ20' on page 8 undefined on input l
ine 126.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-1712-09124' on page 8 undefined
 on input line 126.


LaTeX Warning: Citation 'DBLP:conf/www/Grgic-HlacaRGW18' on page 8 undefined on
 input line 128.


Overfull \hbox (30.6207pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) place [[]] or fur-ther con-firm the stereo
-types [[],

Overfull \hbox (142.4989pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) agents tend to under-monitor when they per
-ceive affin-ity to-wards the mon-i-tor case at hand [[]],

Overfull \hbox (14.24838pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) or sim-ply when they deem their rea-son-in
g more ``hu-man'' than the ma-chine's [[]].

Overfull \hbox (38.19225pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) decision-making of the hu-man agents [[], 
[]].

LaTeX Warning: Citation 'englich2006playing' on page 8 undefined on input line 
132.


Overfull \hbox (2.2601pt too wide) in paragraph at lines 132--132
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 132--132
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

LaTeX Warning: Citation 'DBLP:journals/corr/abs-1812-03219' on page 8 undefined
 on input line 134.


LaTeX Warning: Citation 'albright2019if' on page 8 undefined on input line 134.



LaTeX Warning: Citation 'DBLP:journals/csur/GuidottiMRTGP19' on page 8 undefine
d on input line 140.


LaTeX Warning: Citation 'DBLP:conf/nips/LundbergL17' on page 8 undefined on inp
ut line 141.


LaTeX Warning: Citation 'DBLP:journals/expert/GuidottiMGPRT19' on page 8 undefi
ned on input line 141.


LaTeX Warning: Citation 'DBLP:conf/icml/KohL17' on page 8 undefined on input li
ne 141.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-2303-09297' on page 8 undefined
 on input line 141.


Overfull \hbox (80.86664pt too wide) in paragraph at lines 138--143
\T1/LinuxLibertineT-TLF/m/n/10 (-20) to fur-ther ex-plain the pre-dic-tions giv
en by a ma-chine. Ex-plain-able AI (XAI) [[]]
)

LaTeX Warning: Citation 'cortes2016l2r' on page 8 undefined on input line 273.

[8.8]

LaTeX Warning: Citation 'Chow1970' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'cortes2016l2r' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'Madras18' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'Mozannar20' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'Madras18' on page 9 undefined on input line 285.

(./L2R.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (9.70471pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dovremmo 

Overfull \hbox (9.31847pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigma 

Overfull \hbox (8.02188pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) vazionalei[]  

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (9.70471pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dovremmo 

Overfull \hbox (9.31847pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigma 

Overfull \hbox (8.02188pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) vazionalei[]  

LaTeX Warning: Citation 'Chow1970' on page 9 undefined on input line 3.


LaTeX Warning: Citation 'Chow1970' on page 9 undefined on input line 3.


LaTeX Warning: Citation 'ZhangSurv' on page 9 undefined on input line 6.


LaTeX Warning: Citation 'el_yaniv_foundation' on page 9 undefined on input line
 6.


LaTeX Warning: Citation 'HendrickxSurv' on page 9 undefined on input line 6.


LaTeX Warning: Citation 'HendrickxSurv' on page 9 undefined on input line 9.


LaTeX Warning: Citation 'HendrickxSurv' on page 9 undefined on input line 9.


LaTeX Warning: Citation 'ZhangSurv' on page 9 undefined on input line 9.


LaTeX Warning: Citation 'ZhangSurv' on page 9 undefined on input line 9.

[9.9]

LaTeX Warning: Citation 'GyorfiBayes' on page 10 undefined on input line 35.


LaTeX Warning: Citation 'outlier_survey_2004' on page 10 undefined on input lin
e 45.


LaTeX Warning: Citation 'anomaly_comprehensive_2020' on page 10 undefined on in
put line 45.


LaTeX Warning: Citation 'openset_surv' on page 10 undefined on input line 45.


Overfull \hbox (32.09886pt too wide) in paragraph at lines 45--46
\T1/LinuxLibertineT-TLF/m/it/10 (-20) tions\T1/LinuxLibertineT-TLF/m/n/10 (-20)
 . Most of the works in this par-tic-u-lar area frame the prob-lem as \T1/Linux
LibertineT-TLF/m/it/10 (-20) Out-lier de-tec-tion \T1/LinuxLibertineT-TLF/m/n/1
0 (-20) [[]]

LaTeX Warning: Citation 'Seo_Wallat_Graepel_Obermayer_2000' on page 10 undefine
d on input line 47.


LaTeX Warning: Citation 'Seo_Wallat_Graepel_Obermayer_2000' on page 10 undefine
d on input line 47.


LaTeX Warning: Citation 'Coles2001' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'Coles2001' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'Scheirer11' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'math11092171' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'ruddEVM' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'ruddEVM' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'vignotto_extreme_2020' on page 10 undefined on input l
ine 47.


Overfull \hbox (74.74547pt too wide) in paragraph at lines 47--48
\T1/LinuxLibertineT-TLF/m/n/10 (-20) cesses as a test-ing point to un-der-stand
 whether to re-ject a data point or not [[]].
[10.10]

LaTeX Warning: Citation 'Coenen2020ProbabilityOD' on page 11 undefined on input
 line 49.


LaTeX Warning: Citation 'Coenen2020ProbabilityOD' on page 11 undefined on input
 line 49.


LaTeX Warning: Citation 'Landgrebe' on page 11 undefined on input line 49.


LaTeX Warning: Citation 'fewshotanom' on page 11 undefined on input line 49.


LaTeX Warning: Citation 'AsifNets' on page 11 undefined on input line 51.


LaTeX Warning: Citation 'AsifNets' on page 11 undefined on input line 51.


LaTeX Warning: Citation 'Dalitz2009RejectOA' on page 11 undefined on input line
 55.


LaTeX Warning: Citation 'Grandvalet2008' on page 11 undefined on input line 55.



LaTeX Warning: Citation 'Jnior2017NearestND' on page 11 undefined on input line
 55.


LaTeX Warning: Citation 'hansen_error_reject_1997' on page 11 undefined on inpu
t line 62.


LaTeX Warning: Citation 'el_yaniv_foundation' on page 11 undefined on input lin
e 62.


Overfull \hbox (3.87013pt too wide) in paragraph at lines 60--66
\T1/LinuxLibertineT-TLF/m/n/10 (-20) tion $\OML/nxlmi/m/it/10 f$\T1/LinuxLibert
ineT-TLF/m/n/10 (-20) , and $\OML/nxlmi/m/it/10 ^^\$ \T1/LinuxLibertineT-TLF/m/
n/10 (-20) is the thresh-old hy-per-pa-ram-e-ter [[], []].

LaTeX Warning: Citation 'battisti_democracy' on page 11 undefined on input line
 68.


LaTeX Warning: Citation 'sousa_map' on page 11 undefined on input line 68.


Overfull \hbox (20.76775pt too wide) in paragraph at lines 68--69
\T1/LinuxLibertineT-TLF/m/n/10 (-20) sider the class-wise vari-ance of these pr
e-dic-tions as in-di-ca-tion of un-cer-tainty [[],

LaTeX Warning: Citation 'destefano_shakespear' on page 11 undefined on input li
ne 69.


LaTeX Warning: Citation 'brinkrolf_lvq' on page 11 undefined on input line 69.


LaTeX Warning: Citation 'tortorella_svm' on page 11 undefined on input line 73.



LaTeX Warning: Citation 'tortorella_svm' on page 11 undefined on input line 73.



LaTeX Warning: Citation 'Johannes_interpretable_conf' on page 11 undefined on i
nput line 74.

[11.11]

LaTeX Warning: Citation 'capitaine_frelicot' on page 12 undefined on input line
 76.


LaTeX Warning: Citation 'ceccotti_vajda' on page 12 undefined on input line 76.



LaTeX Warning: Citation 'Fischer_multiple_tau' on page 12 undefined on input li
ne 77.


LaTeX Warning: Citation 'pillai' on page 12 undefined on input line 77.


LaTeX Warning: Citation 'Fischer_variance' on page 12 undefined on input line 7
7.


Overfull \hbox (2.31824pt too wide) in paragraph at lines 76--78
\T1/LinuxLibertineT-TLF/m/n/10 (-20) [[], []]. Mul-ti-ple lo-cal thresh-olds $\
OML/nxlmi/m/it/10 ^^\[]; [] ; ^^\[]$ \T1/LinuxLibertineT-TLF/m/n/10 (-20) [[]]

LaTeX Warning: Citation 'HendrickxSurv' on page 12 undefined on input line 79.


LaTeX Warning: Citation 'cortes2016l2r' on page 12 undefined on input line 79.


LaTeX Warning: Citation 'Bartlett2008' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'RamaswamyReject' on page 12 undefined on input line 80
.


LaTeX Warning: Citation 'pugnana2023' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'pugnana2023' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'Ziyin2019' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'Grandvalet2008' on page 12 undefined on input line 81.



LaTeX Warning: Citation 'LIN2018' on page 12 undefined on input line 81.


LaTeX Warning: Citation 'Geifman2019SelectiveNetAD' on page 12 undefined on inp
ut line 81.


LaTeX Warning: Citation 'cortes2016l2r' on page 12 undefined on input line 86.


LaTeX Warning: Citation 'cortes2016l2r' on page 12 undefined on input line 86.

(/usr/share/texmf-dist/tex/latex/bbm-macros/ubbm.fd)

LaTeX Font Warning: Font shape `U/bbm/m/n' in size <5.5> not available
(Font)              size <5> substituted on input line 103.


LaTeX Warning: Citation 'Geifman2019SelectiveNetAD' on page 12 undefined on inp
ut line 109.

[12.12]

LaTeX Warning: Citation 'GeifmanNIPS17' on page 13 undefined on input line 111.



LaTeX Warning: Citation 'GeifmanNIPS17' on page 13 undefined on input line 111.



LaTeX Warning: Citation 'pmlr-v97-franc19a' on page 13 undefined on input line 
126.


LaTeX Warning: Citation 'JonesSKKL21' on page 13 undefined on input line 129.

) (./L2D.tex [13.13]

LaTeX Warning: Citation 'cortes2016l2r' on page 14 undefined on input line 75.


LaTeX Warning: Citation 'Madras18' on page 14 undefined on input line 77.


LaTeX Warning: Citation 'De2020Class' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Mozannar20' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Mozannar2023' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Okati2021' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Keswani2021' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Madras18' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Mozannar2023' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Martinez20' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Raghu2019TheAA' on page 14 undefined on input line 113
.


LaTeX Warning: Citation 'Verma2022Multi' on page 14 undefined on input line 128
.

[14.14]

LaTeX Warning: Citation 'Raghu2019TheAA' on page 15 undefined on input line 151
.


LaTeX Warning: Citation 'Raghu2019Med' on page 15 undefined on input line 152.


LaTeX Warning: Citation 'Bansal2021IsTM' on page 15 undefined on input line 156
.


LaTeX Warning: Citation 'Wilder2020' on page 15 undefined on input line 161.


LaTeX Warning: Citation 'Charusaie2022' on page 15 undefined on input line 164.



LaTeX Warning: Citation 'Charusaie2022' on page 15 undefined on input line 165.



LaTeX Warning: Citation 'Mozannar2023' on page 15 undefined on input line 173.


LaTeX Warning: Citation 'Mozannar2023' on page 15 undefined on input line 173.


Class acmart Warning: A possible image without description on input line 175.

[15.15]

LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 206.


LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 206.


LaTeX Warning: Citation 'Lin2004' on page 16 undefined on input line 210.


LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 211.


LaTeX Warning: Citation 'Charusaie2022' on page 16 undefined on input line 211.



LaTeX Warning: Citation 'Verma22' on page 16 undefined on input line 211.


LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 212.


LaTeX Warning: Citation 'Charusaie2022' on page 16 undefined on input line 217.


[16.16 <./media/joint_deferral_content_moderation.png>]

LaTeX Warning: Citation 'Liu2022' on page 17 undefined on input line 225.


LaTeX Warning: Citation 'Raman2021' on page 17 undefined on input line 226.


LaTeX Warning: Citation 'Dawid1982' on page 17 undefined on input line 229.


LaTeX Warning: Citation 'Verma22' on page 17 undefined on input line 229.


LaTeX Warning: Citation 'Verma22' on page 17 undefined on input line 229.


LaTeX Warning: Citation 'Bansal2021IsTM' on page 17 undefined on input line 234
.


LaTeX Warning: Citation 'Mozannar20' on page 17 undefined on input line 234.


LaTeX Warning: Citation 'Okati2021' on page 17 undefined on input line 234.


LaTeX Warning: Citation 'Raghu2019TheAA' on page 17 undefined on input line 234
.


LaTeX Warning: Citation 'Mozannar2023' on page 17 undefined on input line 237.


LaTeX Warning: Citation 'Madras18' on page 17 undefined on input line 249.


LaTeX Warning: Citation 'Mozannar20' on page 17 undefined on input line 249.


LaTeX Warning: Citation 'Pradier2021' on page 17 undefined on input line 250.


LaTeX Warning: Citation 'Madras18' on page 17 undefined on input line 250.

[17.17]

LaTeX Warning: Citation 'Wilder2020' on page 18 undefined on input line 255.


LaTeX Warning: Citation 'Mozannar2023' on page 18 undefined on input line 257.


LaTeX Warning: Citation 'Hemmer2022' on page 18 undefined on input line 285.


LaTeX Warning: Citation 'Verma2022Multi' on page 18 undefined on input line 287
.


LaTeX Warning: Citation 'Hemmer2022' on page 18 undefined on input line 289.


LaTeX Warning: Citation 'Gao2021' on page 18 undefined on input line 291.


LaTeX Warning: Citation 'Keswani2021' on page 18 undefined on input line 305.

[18.18]

LaTeX Warning: Citation 'Keswani2022' on page 19 undefined on input line 316.


LaTeX Warning: Citation 'Verma2022Multi' on page 19 undefined on input line 323
.


LaTeX Warning: Citation 'Shafer2008' on page 19 undefined on input line 323.


LaTeX Warning: Citation 'Angelopoulos2022' on page 19 undefined on input line 3
23.


LaTeX Warning: Citation 'Okati2021' on page 19 undefined on input line 329.


LaTeX Warning: Citation 'Mozannar2023' on page 19 undefined on input line 329.


LaTeX Warning: Citation 'De2020Class' on page 19 undefined on input line 331.


LaTeX Warning: Citation 'De2020Reg' on page 19 undefined on input line 331.


LaTeX Warning: Citation 'Leitao2022' on page 19 undefined on input line 342.


LaTeX Warning: Citation 'Hemmer2023' on page 19 undefined on input line 342.


LaTeX Warning: Citation 'Charusaie2022' on page 19 undefined on input line 344.



LaTeX Warning: Citation 'Cohn1994' on page 19 undefined on input line 344.

[19.19]

LaTeX Warning: Citation 'Hemmer2023' on page 20 undefined on input line 347.


LaTeX Warning: Citation 'Hemmer2023UserStudy' on page 20 undefined on input lin
e 359.


LaTeX Warning: Citation 'Papenmeier2023' on page 20 undefined on input line 362
.


LaTeX Warning: Citation 'Leitao2022' on page 20 undefined on input line 367.


LaTeX Warning: Citation 'Jones21' on page 20 undefined on input line 368.

[20.20]) (./human_interaction.tex

LaTeX Warning: Citation 'DBLP:journals/nn/VapnikV09' on page 21 undefined on in
put line 42.


LaTeX Warning: Citation 'DBLP:conf/kdd/BucilaCN06' on page 21 undefined on inpu
t line 42.


LaTeX Warning: Citation 'DBLP:journals/pieee/ZhuangQDXZZXH21' on page 21 undefi
ned on input line 42.


LaTeX Warning: Citation 'settles2009active' on page 21 undefined on input line 
42.


Overfull \hbox (43.57573pt too wide) in paragraph at lines 42--49
\T1/LinuxLibertineT-TLF/m/n/10 (-20) Trans-fer Learn-ing [[]], and Ac-tive Lear
n-ing [[]].

LaTeX Warning: Citation 'DBLP:journals/nn/VapnikV09' on page 21 undefined on in
put line 50.

[21.21]

LaTeX Warning: Citation 'DBLP:conf/kdd/BucilaCN06' on page 22 undefined on inpu
t line 70.


LaTeX Warning: Citation 'DBLP:journals/pieee/ZhuangQDXZZXH21' on page 22 undefi
ned on input line 93.


Overfull \hbox (149.376pt too wide) in paragraph at lines 93--97
\T1/LinuxLibertineT-TLF/m/n/10 (-20) tries to lever-age the knowl-edge of the T
eacher, and only then adapts it to the task at hand [[]].

LaTeX Warning: Citation 'settles2009active' on page 22 undefined on input line 
103.


LaTeX Warning: Citation 'settles2009active' on page 22 undefined on input line 
119.


LaTeX Warning: Citation 'DBLP:conf/nldb/MullerPBF22' on page 22 undefined on in
put line 119.


LaTeX Warning: Citation 'DBLP:journals/ml/CohnAL94' on page 22 undefined on inp
ut line 119.


LaTeX Warning: Citation 'DBLP:journals/ml/CohnAL94' on page 22 undefined on inp
ut line 120.

[22.22{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_kijugd.enc}]
[23.23]
Overfull \hbox (2.2601pt too wide) in paragraph at lines 214--214
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 214--214
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (5.42758pt too wide) in paragraph at lines 216--216
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) Abbiamo 

Overfull \hbox (1.56297pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) roberto 

Overfull \hbox (8.2248pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigmi 

Overfull \hbox (5.7366pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) rezionale 

Overfull \hbox (1.65099pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) sezione 

Overfull \hbox (14.38783pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) l'importanza 

Overfull \hbox (4.70122pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) fragilita', 

Overfull \hbox (5.42758pt too wide) in paragraph at lines 216--216
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) Abbiamo 

Overfull \hbox (1.56297pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) roberto 

Overfull \hbox (8.2248pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigmi 

Overfull \hbox (5.7366pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) rezionale 

Overfull \hbox (1.65099pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) sezione 

Overfull \hbox (14.38783pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) l'importanza 

Overfull \hbox (4.70122pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) fragilita', 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 217--217
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (5.5602pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) nell'altro 

Overfull \hbox (3.52669pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) munque 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 217--217
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (5.5602pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) nell'altro 

Overfull \hbox (3.52669pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) munque 

LaTeX Warning: Marginpar on page 24 moved.


LaTeX Warning: Marginpar on page 24 moved.


Underfull \hbox (badness 10000) in paragraph at lines 219--222


Overfull \hbox (2.2601pt too wide) in paragraph at lines 244--244
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.4399pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) mento? 

Overfull \hbox (5.03302pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) potrebbe 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 244--244
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.4399pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) mento? 

Overfull \hbox (5.03302pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) potrebbe 

LaTeX Warning: Marginpar on page 24 moved.


Underfull \hbox (badness 10000) in paragraph at lines 259--269

[24.24]

Class acmart Warning: A possible image without description on input line 297.


LaTeX Warning: Citation 'DBLP:conf/cvpr/JohnsonHMFZG17' on page 25 undefined on
 input line 299.


LaTeX Warning: Citation 'DBLP:conf/iui/GuoDAMCK22' on page 25 undefined on inpu
t line 304.


LaTeX Warning: Citation 'DBLP:conf/pldi/EllisWNSMHCST21' on page 25 undefined o
n input line 312.

[25.25]

LaTeX Warning: Citation 'DBLP:conf/emnlp/KassnerTSC21' on page 26 undefined on 
input line 336.


LaTeX Warning: Citation 'DBLP:conf/nips/LewisPPPKGKLYR020' on page 26 undefined
 on input line 336.


LaTeX Warning: Citation 'DBLP:conf/ijcai/ClarkTR20' on page 26 undefined on inp
ut line 336.


Overfull \hbox (35.3791pt too wide) in paragraph at lines 336--343
\T1/LinuxLibertineT-TLF/m/n/10 (-20) builds on top of two other fam-i-lies, kno
wl-edge in-jec-tion mod-els [[]]

LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 380.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 380.


Class acmart Warning: A possible image without description on input line 382.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 384.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 390.


LaTeX Warning: Citation 'DBLP:conf/emnlp/BostromZCD21' on page 26 undefined on 
input line 392.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MurtyMLR22' on page 26 undefined on in
put line 393.


LaTeX Warning: Citation 'DBLP:conf/nips/LewisPPPKGKLYR020' on page 26 undefined
 on input line 404.


LaTeX Warning: Citation 'DBLP:conf/aaai/HwangBBDSBC21' on page 26 undefined on 
input line 406.


LaTeX Warning: Citation 'DBLP:journals/cacm/VrandecicK14' on page 26 undefined 
on input line 406.


LaTeX Warning: Citation 'wang2017fvqa' on page 26 undefined on input line 431.

[26.26 <./media/clever.pdf>]

LaTeX Warning: Citation 'MalandriMMN23' on page 27 undefined on input line 457.



LaTeX Warning: Citation 'DBLP:journals/aim/AmershiCKK14' on page 27 undefined o
n input line 463.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 27 undefined on input 
line 463.

[27.27]
Overfull \hbox (2.2601pt too wide) in paragraph at lines 489--489
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.90285pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) lascerei 

Overfull \hbox (3.19742pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tostante 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 489--489
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.90285pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) lascerei 

Overfull \hbox (3.19742pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tostante 

LaTeX Warning: Citation 'DBLP:conf/ijcai/RossHD17' on page 28 undefined on inpu
t line 493.


LaTeX Warning: Citation 'teso2019toward' on page 28 undefined on input line 493
.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 28 undefined on input 
line 493.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 28 undefined on input 
line 504.


LaTeX Warning: Citation 'DBLP:conf/kdd/WangKNSNCVV022' on page 28 undefined on 
input line 506.

[28.28 <./media/hydrant_only.png>]

LaTeX Warning: Citation 'Popordanoska2020' on page 29 undefined on input line 5
12.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-2012-02898' on page 29 undefine
d on input line 514.


Overfull \hbox (40.68759pt too wide) in paragraph at lines 511--515
\T1/LinuxLibertineT-TLF/m/n/10 (-20) the cor-rec-tion is again an added com-po-
nent of the ma-chine ob-jec-tive [[]]. 

LaTeX Warning: Citation 'DBLP:journals/datamine/BontempelliGPT22' on page 29 un
defined on input line 517.

[29.29])
Overfull \hbox (9.70557pt too wide) in paragraph at lines 305--305
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) richiamare 

Overfull \hbox (9.70557pt too wide) in paragraph at lines 305--305
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) richiamare 

LaTeX Warning: Citation 'Sarkar2023' on page 30 undefined on input line 312.

[30.30] (./conclusions.tex)

LaTeX Warning: Empty bibliography on input line 338.

[31.31] (./appendices.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (6.47256pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tosezione 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (6.47256pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tosezione 

LaTeX Warning: Citation 'Fisher1922' on page 32 undefined on input line 7.


LaTeX Warning: Citation 'Lin2004' on page 32 undefined on input line 8.


LaTeX Warning: Citation 'Bartlett2006' on page 32 undefined on input line 8.


LaTeX Warning: Citation 'Long2013' on page 32 undefined on input line 12.


LaTeX Warning: Citation 'Mozannar2023' on page 32 undefined on input line 14.


LaTeX Warning: Citation 'Verma22' on page 32 undefined on input line 14.


LaTeX Warning: Citation 'Lin2004' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Liu2007' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Tewari2007' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Zou2008' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Mozannar20' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Verma22' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Fisher1922' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Gerow1989' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Bartlett2006' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Lin2004' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Neykov2016' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Steinwart2007' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Tewari2007' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Bartlett2006' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Dawid1982' on page 32 undefined on input line 22.


LaTeX Warning: Citation 'Verma22' on page 32 undefined on input line 22.


LaTeX Warning: Citation 'Vaicenavicius2019' on page 32 undefined on input line 
22.


LaTeX Warning: Citation 'SilvaFilho2023' on page 32 undefined on input line 25.



LaTeX Warning: Citation 'Vaicenavicius2019' on page 32 undefined on input line 
29.


LaTeX Warning: Citation 'Kull2019' on page 32 undefined on input line 30.


LaTeX Warning: Citation 'SilvaFilho2023' on page 32 undefined on input line 30.


[32.32]

LaTeX Warning: Citation 'Verma2022Multi' on page 33 undefined on input line 32.



LaTeX Warning: Citation 'Verma22' on page 33 undefined on input line 32.


LaTeX Warning: Citation 'Verma22' on page 33 undefined on input line 40.


LaTeX Warning: Citation 'Verma2022Multi' on page 33 undefined on input line 40.



LaTeX Warning: Citation 'Long2013' on page 33 undefined on input line 46.


LaTeX Warning: Citation 'Long2013' on page 33 undefined on input line 46.


LaTeX Warning: Citation 'cortes2016l2r' on page 33 undefined on input line 47.


LaTeX Warning: Citation 'Mozannar20' on page 33 undefined on input line 47.


LaTeX Warning: Citation 'Mozannar2023' on page 33 undefined on input line 47.


LaTeX Warning: Citation 'cortes2016l2r' on page 33 undefined on input line 50.


LaTeX Warning: Citation 'Mozannar2023' on page 33 undefined on input line 50.


LaTeX Warning: Citation 'Mozannar20' on page 33 undefined on input line 50.


LaTeX Warning: Citation 'Mozannar2023' on page 33 undefined on input line 64.

[33.33] [34.34]
Overfull \hbox (10.90298pt too wide) in paragraph at lines 92--92
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Architecture| 

Overfull \hbox (5.88702pt too wide) in paragraph at lines 92--92
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Theoretical

Underfull \hbox (badness 10000) in paragraph at lines 92--92
\T1/LinuxLibertineT-TLF/m/n/10 (+20) guar-an-

Overfull \hbox (26.71838pt too wide) in paragraph at lines 92--92
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Constraints| 

LaTeX Warning: Citation 'Raghu2019TheAA' on page 35 undefined on input line 93.



Overfull \hbox (2.99666pt too wide) in paragraph at lines 93--93
[]|[]| 

Overfull \hbox (8.51001pt too wide) in paragraph at lines 93--93
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Budget| 

Underfull \hbox (badness 10000) in paragraph at lines 93--93
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Retinal

Underfull \hbox (badness 10000) in paragraph at lines 93--93
\T1/LinuxLibertineT-TLF/m/n/10 (+20) fun-dus

Underfull \hbox (badness 10000) in paragraph at lines 93--93
\T1/LinuxLibertineT-TLF/m/n/10 (+20) pho-

LaTeX Warning: Citation 'Wilder2020' on page 35 undefined on input line 94.


Underfull \hbox (badness 10000) in paragraph at lines 94--94
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Staged,

Underfull \hbox (badness 10000) in paragraph at lines 94--94
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 94--94
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy

Underfull \hbox (badness 10000) in paragraph at lines 94--94
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Zoo,

Underfull \hbox (badness 10000) in paragraph at lines 94--94
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Breast

LaTeX Warning: Citation 'Bansal2021IsTM' on page 35 undefined on input line 95.



Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) man

Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) credit,

Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) FICO,

Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Com-pas,

LaTeX Warning: Citation 'Madras18' on page 35 undefined on input line 96.


Underfull \hbox (badness 10000) in paragraph at lines 96--96
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Joint

Overfull \hbox (14.13278pt too wide) in paragraph at lines 96--96
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Fairness,

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Cov-

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) er-

Underfull \hbox (badness 10000) in paragraph at lines 96--96
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Com-pas,

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Her-itage

LaTeX Warning: Citation 'Mozannar20' on page 35 undefined on input line 97.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 97--97
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) , CI-

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) FAR10H,

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CheX-

Overfull \hbox (22.41237pt too wide) in paragraph at lines 97--98
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/clinicalml/learn-

LaTeX Warning: Citation 'Verma22' on page 35 undefined on input line 98.


Overfull \hbox (8.51001pt too wide) in paragraph at lines 98--98
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Budget| 

Underfull \hbox (badness 10000) in paragraph at lines 98--98
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 10,

Overfull \hbox (6.44347pt too wide) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (-20) HAM10000,

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy-

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Zoo,

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate-

Overfull \hbox (5.80733pt too wide) in paragraph at lines 98--99
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/rajevv/OvA-

LaTeX Warning: Citation 'Charusaie2022' on page 35 undefined on input line 99.


Underfull \hbox (badness 10000) in paragraph at lines 99--99
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Lim-ited

Underfull \hbox (badness 10000) in paragraph at lines 99--99
\T1/LinuxLibertineT-TLF/m/n/10 (+20) hu-man

Underfull \hbox (badness 10000) in paragraph at lines 99--99
\T1/LinuxLibertineT-TLF/m/n/10 (+20) pre-dic-

Underfull \hbox (badness 10000) in paragraph at lines 99--99
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Overfull \hbox (87.11462pt too wide) in paragraph at lines 99--100
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/clinicalml/active_le
arn_to_defer| 

LaTeX Warning: Citation 'Liu2022' on page 35 undefined on input line 100.


Underfull \hbox (badness 10000) in paragraph at lines 100--100
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 100--100
\T1/LinuxLibertineT-TLF/m/n/10 (+20) MIMIC-

Underfull \hbox (badness 10000) in paragraph at lines 100--100
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Her-itage,

Underfull \hbox (badness 10000) in paragraph at lines 100--100
\T1/LinuxLibertineT-TLF/m/n/10 (+20) MIMIC-

Underfull \hbox (badness 10000) in paragraph at lines 100--101
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) https://github.com/liu-

Underfull \hbox (badness 10000) in paragraph at lines 100--101
\T1/LinuxLibertineT-TLF/m/n/10 (+20) res/Learning-to-Defer-with-

LaTeX Warning: Citation 'Raman2021' on page 35 undefined on input line 101.


Underfull \hbox (badness 10000) in paragraph at lines 101--101
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Synthetic

Underfull \hbox (badness 10000) in paragraph at lines 101--101
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

LaTeX Warning: Citation 'Pradier2021' on page 35 undefined on input line 102.


Underfull \hbox (badness 10000) in paragraph at lines 102--102
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Joint

Overfull \hbox (12.5326pt too wide) in paragraph at lines 102--102
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Sparsity

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) of

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) the

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) de-

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) fer-

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) ral

LaTeX Warning: Citation 'Mozannar2023' on page 35 undefined on input line 103.


Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Lim-ited

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) hu-man

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) pre-dic-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) tions,

Overfull \hbox (14.13278pt too wide) in paragraph at lines 103--103
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Fairness,

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Cov-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) er-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 10H,

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Speach,

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Com-pas,

Overfull \hbox (5.06406pt too wide) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (-20) ChestXRay| 

Overfull \hbox (76.16968pt too wide) in paragraph at lines 103--104
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/clinicalml/human_ai_
deferral| 

LaTeX Warning: Citation 'Okati2021' on page 35 undefined on input line 104.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 104--104
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 104--104
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 104--104
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy-

Underfull \hbox (badness 10000) in paragraph at lines 104--105
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-11) https://github.com/Networks-

Underfull \hbox (badness 10000) in paragraph at lines 104--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Learning/differentiable-

LaTeX Warning: Citation 'De2020Class' on page 35 undefined on input line 105.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 105--105
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 105--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 105--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Stare,

Underfull \hbox (badness 10000) in paragraph at lines 105--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Mes-si-dor,

Underfull \hbox (badness 10000) in paragraph at lines 105--106
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-11) https://github.com/Networks-

Underfull \hbox (badness 10000) in paragraph at lines 105--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Learning/classification-

LaTeX Warning: Citation 'De2020Reg' on page 35 undefined on input line 106.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 106--106
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Speech,

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Stare-H,

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Stare-D,

Underfull \hbox (badness 10000) in paragraph at lines 106--107
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-11) https://github.com/Networks-

Underfull \hbox (badness 10000) in paragraph at lines 106--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Learning/regression-under-

LaTeX Warning: Citation 'Hemmer2023' on page 35 undefined on input line 107.


Underfull \hbox (badness 10000) in paragraph at lines 107--107
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Limited

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hu-man

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Pre-dic-

Underfull \hbox (badness 10000) in paragraph at lines 107--107
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 100,

Overfull \hbox (5.06406pt too wide) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (-20) ChestXRay| 

Overfull \hbox (41.64806pt too wide) in paragraph at lines 107--108
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/ptrckhmmr/learning-

Underfull \hbox (badness 10000) in paragraph at lines 107--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) to-deferwith-limited-expert-

LaTeX Warning: Citation 'Hemmer2022' on page 35 undefined on input line 108.


Underfull \hbox (badness 10000) in paragraph at lines 108--108
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Speech,

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 100,

Overfull \hbox (5.06406pt too wide) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (-20) ChestXRay| 

Overfull \hbox (36.38547pt too wide) in paragraph at lines 108--109
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/ptrckhmmr/human-

LaTeX Warning: Citation 'Verma2022Multi' on page 35 undefined on input line 109
.


Underfull \hbox (badness 4846) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) of J,

Underfull \hbox (badness 10000) in paragraph at lines 109--109
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Overfull \hbox (6.44347pt too wide) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (-20) HAM10000,

Underfull \hbox (badness 10000) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy-

Underfull \hbox (badness 10000) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Zoo,

Underfull \hbox (badness 10000) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate-

Overfull \hbox (29.51352pt too wide) in paragraph at lines 109--110
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/rajevv/Multi_L2D| 

LaTeX Warning: Citation 'Gao2021' on page 35 undefined on input line 110.


Underfull \hbox (badness 10000) in paragraph at lines 110--110
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Staged,

Underfull \hbox (badness 10000) in paragraph at lines 110--110
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 110--110
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Scene,

Underfull \hbox (badness 10000) in paragraph at lines 110--110
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Yeast,

Underfull \hbox (badness 10000) in paragraph at lines 110--110
\T1/LinuxLibertineT-TLF/m/n/10 (+20) MLC,

Overfull \hbox (16.05214pt too wide) in paragraph at lines 110--111
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/ruijiang81/hai-

LaTeX Warning: Citation 'Keswani2021' on page 35 undefined on input line 111.


Overfull \hbox (14.13278pt too wide) in paragraph at lines 111--111
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Fairness,

Overfull \hbox (6.3736pt too wide) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (-20) Sparse

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) com-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) mit-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) tee,

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hu-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) man

Overfull \hbox (13.12315pt too wide) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (-20) dropout,

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hu-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) man

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate

Overfull \hbox (48.74487pt too wide) in paragraph at lines 111--112
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/vijaykeswani/Deferra
l-

LaTeX Warning: Citation 'Keswani2022' on page 35 undefined on input line 112.


Underfull \hbox (badness 10000) in paragraph at lines 112--112
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Joint,

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Lim-ited

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) ground

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Twit-ter

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Eng-lish

Overfull \hbox (42.84532pt too wide) in paragraph at lines 112--113
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/vijaykeswani/Online-

[35.35] [36.36] [37.37] [38.38]
(/usr/share/texmf-dist/tex/generic/stringenc/se-pdfdoc.def)
(/usr/share/texmf-dist/tex/generic/stringenc/se-utf8.def) [39.39])

LaTeX Warning: Empty bibliography on input line 348.


Class acmart Warning: Some images may lack descriptions.

(./main.aux (./appendices.aux))

LaTeX Font Warning: Size substitutions with differences
(Font)              up to 0.5pt have occurred.


LaTeX Warning: There were undefined references.


LaTeX Warning: Label(s) may have changed. Rerun to get cross-references right.


Package rerunfilecheck Warning: File `main.out' has changed.
(rerunfilecheck)                Rerun to get outlines right
(rerunfilecheck)                or use package `bookmark'.


Package biblatex Warning: Please (re)run Biber on the file:
(biblatex)                main
(biblatex)                and rerun LaTeX afterwards.

 )
(see the transcript file for additional information) </home/aslan/.texlive/texm
f-var/fonts/pk/ljfour/public/bbm/bbm10.600pk></usr/share/texmf-dist/fonts/type1
/public/newtx/LibertineMathMI.pfb></usr/share/texmf-dist/fonts/type1/public/new
tx/LibertineMathMI5.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/Liberti
neMathMI7.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/LibertineMathRM.p
fb></usr/share/texmf-dist/fonts/type1/public/libertine/LinBiolinumT.pfb></usr/s
hare/texmf-dist/fonts/type1/public/libertine/LinBiolinumTB.pfb></usr/share/texm
f-dist/fonts/type1/public/libertine/LinBiolinumTI.pfb></usr/share/texmf-dist/fo
nts/type1/public/libertine/LinLibertineT.pfb></usr/share/texmf-dist/fonts/type1
/public/libertine/LinLibertineTB.pfb></usr/share/texmf-dist/fonts/type1/public/
libertine/LinLibertineTBI.pfb></usr/share/texmf-dist/fonts/type1/public/liberti
ne/LinLibertineTI.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/NewTXMI.p
fb></usr/share/texmf-dist/fonts/type1/public/newtx/NewTXMI7.pfb></usr/share/tex
mf-dist/fonts/type1/public/newtx/stxscr.pfb></usr/share/texmf-dist/fonts/type1/
public/newtx/txexas.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/txexs.p
fb></usr/share/texmf-dist/fonts/type1/public/newtx/txmiaX.pfb></usr/share/texmf
-dist/fonts/type1/public/txfonts/txsyb.pfb></usr/share/texmf-dist/fonts/type1/p
ublic/txfonts/txsyc.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/txsys.p
fb>
Output written on main.pdf (39 pages, 2846312 bytes).
Transcript written on main.log.
This is BibTeX, Version 0.99d (TeX Live 2023/Arch Linux)
The top-level auxiliary file: main.aux
I found no \citation commands---while reading file main.aux
I found no \bibdata command---while reading file main.aux
I found no \bibstyle command---while reading file main.aux
(There were 3 error messages)
This is pdfTeX, Version 3.141592653-2.6-1.40.25 (TeX Live 2023/Arch Linux) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2022-11-01> patch level 1
L3 programming layer <2023-02-22> (./acmart.cls
Document Class: acmart 2022/10/24 v1.88 Typesetting articles for the Associatio
n for Computing Machinery
(/usr/share/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/share/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/share/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/share/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/share/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/share/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/share/texmf-dist/tex/latex/amscls/amsart.cls
Document Class: amsart 2020/05/29 v2.20.6
(/usr/share/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/share/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/share/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/share/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/share/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texmf-dist/tex/latex/refcount/refcount.sty
(/usr/share/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/share/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/share/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/share/texmf-dist/tex/latex/everyshi/everyshi.sty))
(/usr/share/texmf-dist/tex/latex/environ/environ.sty
(/usr/share/texmf-dist/tex/latex/trimspaces/trimspaces.sty))
(/usr/share/texmf-dist/tex/latex/textcase/textcase.sty)
(/usr/share/texmf-dist/tex/latex/hyperxmp/hyperxmp.sty
(/usr/share/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/share/texmf-dist/tex/latex/kvsetkeys/kvsetkeys.sty))
(/usr/share/texmf-dist/tex/generic/pdfescape/pdfescape.sty
(/usr/share/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty))
(/usr/share/texmf-dist/tex/generic/stringenc/stringenc.sty)
(/usr/share/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/share/texmf-dist/tex/latex/ifmtarg/ifmtarg.sty)
(/usr/share/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/ifdraft.sty)
(/usr/share/texmf-dist/tex/generic/iftex/ifluatex.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/share/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/share/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/share/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/share/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texmf-dist/tex/generic/gettitlestring/gettitlestring.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/share/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/share/texmf-dist/tex/latex/url/url.sty)
(/usr/share/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/share/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/share/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/share/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty
(/usr/share/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty)))
(/usr/share/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/share/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/share/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/share/texmf-dist/tex/latex/graphics/mathcolor.ltx))
(/usr/share/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/share/texmf-dist/tex/generic/iftex/ifvtex.sty))
(/usr/share/texmf-dist/tex/latex/ncctools/manyfoot.sty
(/usr/share/texmf-dist/tex/latex/ncctools/nccfoots.sty))
(/usr/share/texmf-dist/tex/generic/pdftex/glyphtounicode.tex)
(/usr/share/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/share/texmf-dist/tex/latex/base/fontenc.sty<<t1.cmap>>)
(/usr/share/texmf-dist/tex/latex/libertine/libertine.sty
(/usr/share/texmf-dist/tex/generic/iftex/ifxetex.sty)
(/usr/share/texmf-dist/tex/latex/base/textcomp.sty)
(/usr/share/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/share/texmf-dist/tex/latex/fontaxes/fontaxes.sty)
(/usr/share/texmf-dist/tex/latex/libertine/LinLibertine_I.tex))
(/usr/share/texmf-dist/tex/latex/inconsolata/zi4.sty
`inconsolata-zi4' v1.12, 2019/05/17 Text macros for Inconsolata (msharpe))
(/usr/share/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.71, 2022/01/16 Math macros based originally on txfonts (msharpe)
(/usr/share/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/share/texmf-dist/tex/generic/kastrup/binhex.tex)
amsthm NOT loaded
) (/usr/share/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texmf-dist/tex/latex/caption/caption3.sty
(/usr/share/texmf-dist/tex/latex/caption/caption-ams-smf.sto)))
(/usr/share/texmf-dist/tex/latex/float/float.sty)
(/usr/share/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment') Excluding comment 'CCSXML'
(/usr/share/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty) Special comment 'acks'
(/usr/share/texmf-dist/tex/latex/libertine/T1LinuxLibertineT-TLF.fd))
(/usr/share/texmf-dist/tex/latex/xargs/xargs.sty)
(/usr/share/texmf-dist/tex/latex/bbm-macros/bbm.sty)
(/usr/share/texmf-dist/tex/latex/optidef/optidef.sty
(/usr/share/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/share/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/share/texmf-dist/tex/latex/xifthen/xifthen.sty)
(/usr/share/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/share/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/share/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def))))
(/usr/share/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/share/texmf-dist/tex/latex/graphics/lscape.sty)
(/usr/share/texmf-dist/tex/latex/tools/longtable.sty)
(/usr/share/texmf-dist/tex/latex/todonotes/todonotes.sty
(/usr/share/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/share/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/share/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.tex)
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def)
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/share/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/share/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfkeyslibraryfiltered.code.te
x)) (/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.def
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-pdf.def)))
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigonometric.code
.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.random.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.comparison.code.te
x) (/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integerarithmetics
.code.tex) (/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfint.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconstruct.code.tex
) (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicstate.code.tex)

(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransformations.code.t
ex) (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathprocessing.code.te
x) (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransparency.code.tex)
 (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.tex)))
(/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.tex)
(/usr/share/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-0-65.sty)
(/usr/share/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-1-18.sty))
(/usr/share/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/share/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex))
(/usr/share/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothandlers.code.te
x) (/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
topaths.code.tex)))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
positioning.code.tex)) (/usr/share/texmf-dist/tex/latex/doublestroke/dsfont.sty
) (/usr/share/texmf-dist/tex/latex/makecell/makecell.sty
(/usr/share/texmf-dist/tex/latex/tools/array.sty))
(/usr/share/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/share/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
arrows.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/pgflibraryarrows.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.geometric.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.geomet
ric.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.misc.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.misc.c
ode.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.symbols.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.symbol
s.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.arrows.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.arrows
.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.callouts.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.callou
ts.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.multipart.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.multip
art.code.tex)))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
calc.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
decorations.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmoduledecorations.code.tex))
(/usr/share/texmf-dist/tex/latex/varwidth/varwidth.sty)
(/usr/share/texmf-dist/tex/latex/biblatex/biblatex.sty
(/usr/share/texmf-dist/tex/latex/logreq/logreq.sty
(/usr/share/texmf-dist/tex/latex/logreq/logreq.def))
(/usr/share/texmf-dist/tex/latex/biblatex/blx-dm.def)
(/usr/share/texmf-dist/tex/latex/biblatex/blx-compat.def)
(/usr/share/texmf-dist/tex/latex/biblatex/biblatex.def)
(/usr/share/texmf-dist/tex/latex/biblatex/blx-natbib.def) (./acmnumeric.bbx
(/usr/share/texmf-dist/tex/latex/biblatex-trad/trad-plain.bbx
(/usr/share/texmf-dist/tex/latex/biblatex-trad/trad-standard.bbx
(/usr/share/texmf-dist/tex/latex/biblatex/bbx/standard.bbx)))
(/usr/share/texmf-dist/tex/latex/biblatex-software/software.bbx
(/usr/share/texmf-dist/tex/latex/xurl/xurl.sty
xurl: Set penalties for biblatex
))) (./acmnumeric.cbx (/usr/share/texmf-dist/tex/latex/biblatex/cbx/numeric.cbx
)) (/usr/share/texmf-dist/tex/latex/biblatex/biblatex.cfg)
(/usr/share/texmf-dist/tex/latex/biblatex/blx-case-expl3.sty))
Excluding comment 'screenonly' Include comment 'printonly'
Include comment 'anonsuppress'

LaTeX Warning: Unused global option(s):
    [natbib=false].

(./main.aux (./appendices.aux))
(/usr/share/texmf-dist/tex/latex/newtx/omlnxlmi.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/share/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/share/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
(/usr/share/texmf-dist/tex/latex/libertine/OT1LinuxLibertineT-TLF.fd)<<ot1.cmap
>><<oml.cmap>> (/usr/share/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxsyc.fd) (./main.out) (./main.out)
(/usr/share/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/share/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/share/texmf-dist/tex/latex/upquote/upquote.sty)
(/usr/share/texmf-dist/tex/latex/caption/ltcaption.sty)

Package todonotes Warning: The length marginparwidth is less than 2cm and will 
most likely cause issues with the appearance of inserted todonotes. The issue c
an be solved by adding a line like \setlength {\marginparwidth }{2cm} prior to 
loading the todonotes package. on input line 144.

(/usr/share/texmf-dist/tex/latex/biblatex/lbx/american.lbx
(/usr/share/texmf-dist/tex/latex/biblatex-software/english-software.lbx
(/usr/share/texmf-dist/tex/latex/biblatex/lbx/english.lbx))
(/usr/share/texmf-dist/tex/latex/biblatex-software/english-software.lbx
(/usr/share/texmf-dist/tex/latex/biblatex/lbx/english.lbx))) (./main.bbl)
Excluding 'CCSXML' comment.
(/usr/share/texmf-dist/tex/latex/libertine/T1LinuxBiolinumT-TLF.fd)
(/usr/share/texmf-dist/tex/latex/libertine/TS1LinuxLibertineT-TLF.fd)
(/usr/share/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/share/texmf-dist/tex/latex/microtype/mt-msb.cfg) (./introduction.tex

LaTeX Warning: Citation 'dietvorst2015algorithm' on page 1 undefined on input l
ine 16.


LaTeX Warning: Citation 'lee2004trust' on page 1 undefined on input line 16.


LaTeX Warning: Citation 'dietvorst2015algorithm' on page 1 undefined on input l
ine 18.


LaTeX Warning: Citation 'logg2019algorithm' on page 1 undefined on input line 1
8.


Overfull \hbox (2.52794pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) assisted 

Overfull \hbox (5.77692pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Decision- 

Overfull \hbox (1.92734pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) making 

Overfull \hbox (3.57817pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Bucinca, 

Overfull \hbox (3.45026pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) man+AI 

Overfull \hbox (1.0689pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dently"[]  

Overfull \hbox (2.52794pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) assisted 

Overfull \hbox (5.77692pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Decision- 

Overfull \hbox (1.92734pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) making 

Overfull \hbox (3.57817pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Bucinca, 

Overfull \hbox (3.45026pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) man+AI 

Overfull \hbox (1.0689pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dently"[]  

LaTeX Warning: Citation 'rajpurkar2022ai' on page 1 undefined on input line 23.



LaTeX Warning: Citation 'goodell2021artificial' on page 1 undefined on input li
ne 23.


LaTeX Warning: Citation 'surden2019artificial' on page 1 undefined on input lin
e 23.


LaTeX Warning: Citation 'DBLP:conf/iclr/Saparov023' on page 1 undefined on inpu
t line 28.


LaTeX Warning: Citation 'DBLP:journals/tkdd/KaufmanRPS12' on page 1 undefined o
n input line 28.


LaTeX Warning: Citation 'DBLP:conf/nips/SolaimanD21' on page 1 undefined on inp
ut line 28.

[1.1{/var/lib/texmf/fonts/map/pdftex/updmap/pdftex.map}{/usr/share/texmf-dist/f
onts/enc/dvips/libertine/lbtn_25tcsq.enc}{/usr/share/texmf-dist/fonts/enc/dvips
/libertine/lbtn_76gpa5.enc}{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbt
n_naooyc.enc}{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_nh77jq.enc}{
/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_7grukw.enc}]

LaTeX Warning: Citation 'DBLP:conf/emnlp/CiosiciCLHFW21' on page 2 undefined on
 input line 51.


LaTeX Warning: Citation 'DBLP:conf/acl/ChenSFC0X23' on page 2 undefined on inpu
t line 51.


LaTeX Warning: Citation 'ferguson2020high' on page 2 undefined on input line 51
.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-1808-09123' on page 2 undefined
 on input line 53.


LaTeX Warning: Citation 'kempt2022m' on page 2 undefined on input line 53.


LaTeX Warning: Citation 'DBLP:conf/ijcai/RossHD17' on page 2 undefined on input
 line 53.


LaTeX Warning: Citation 'hildebrandt2013privacy' on page 2 undefined on input l
ine 56.


LaTeX Warning: Citation 'DBLP:conf/aaai/BansalW18' on page 2 undefined on input
 line 71.


LaTeX Warning: Citation 'DBLP:conf/hcomp/BansalNKLWH19' on page 2 undefined on 
input line 81.


Overfull \hbox (9.47112pt too wide) in paragraph at lines 81--81
\T1/LinuxLibertineT-TLF/m/n/6 (-20) bern[]etik[]es, 

Overfull \hbox (9.47112pt too wide) in paragraph at lines 81--81
\T1/LinuxLibertineT-TLF/m/n/6 (-20) bern[]etik[]es, 

LaTeX Warning: Citation 'dietvorst2018overcoming' on page 2 undefined on input 
line 81.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 2 undefined on input l
ine 82.

[2.2]

LaTeX Warning: Citation 'DBLP:journals/csur/YuZLHWJJ22' on page 3 undefined on 
input line 114.


LaTeX Warning: Citation '10.5555/3312046' on page 3 undefined on input line 114
.


LaTeX Warning: Citation 'DBLP:conf/ijcai/NobaniMM21' on page 3 undefined on inp
ut line 114.


Overfull \hbox (4.55762pt too wide) in paragraph at lines 168--169
 [][] 

Class acmart Warning: A possible image without description on input line 177.

[3.3]) (./paradigms.tex

Package caption Warning: \label without proper reference on input line 5.
See the caption package documentation for explanation.


LaTeX Warning: Reference `tbl:symbols' on page 4 undefined on input line 81.


LaTeX Warning: Citation 'Neykov2016' on page 4 undefined on input line 111.


LaTeX Warning: Citation 'Goodfellow2016' on page 4 undefined on input line 113.



LaTeX Warning: Citation 'Bartlett2006' on page 4 undefined on input line 113.


LaTeX Warning: Citation 'Lin2004' on page 4 undefined on input line 113.

[4.4{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_ki75ao.enc}{/usr/shar
e/texmf-dist/fonts/enc/dvips/libertine/lbtn_oexx6f.enc}] [5.5]

LaTeX Warning: Citation 'Lampert2016' on page 6 undefined on input line 130.


LaTeX Warning: Citation 'Kerrigan2021' on page 6 undefined on input line 132.

) (./human_oversight.tex

LaTeX Warning: Citation 'koulu2020proceduralizing' on page 6 undefined on input
 line 3.


LaTeX Warning: Citation 'quinonero2008dataset' on page 6 undefined on input lin
e 48.


Overfull \hbox (40.22641pt too wide) in paragraph at lines 48--54
[]\T1/LinuxLibertineT-TLF/m/it/10 (-20) Data shift. \T1/LinuxLibertineT-TLF/m/n
/10 (-20) Data shift is gen-er-ally in-tended as a change in the data dis-tri-b
u-tion [[]],
[6.6]

LaTeX Warning: Citation 'DBLP:journals/pacmhci/BucincaMG21' on page 7 undefined
 on input line 64.


LaTeX Warning: Citation 'parikh1994intuition' on page 7 undefined on input line
 67.


LaTeX Warning: Citation 'babuta2021machine' on page 7 undefined on input line 7
9.


LaTeX Warning: Citation 'malgieri2017right' on page 7 undefined on input line 7
9.


LaTeX Warning: Citation 'babuta2021machine' on page 7 undefined on input line 8
3.


LaTeX Warning: Citation 'ferguson2020high' on page 7 undefined on input line 83
.


LaTeX Warning: Citation 'gillespie2018custodians' on page 7 undefined on input 
line 83.


LaTeX Warning: Citation 'DBLP:conf/fat/RaghavanBKL20' on page 7 undefined on in
put line 84.


LaTeX Warning: Citation 'nahmias2021oversight' on page 7 undefined on input lin
e 87.


LaTeX Warning: Citation 'dietvorst2015algorithm' on page 7 undefined on input l
ine 108.


LaTeX Warning: Citation 'logg2019algorithm' on page 7 undefined on input line 1
08.


LaTeX Warning: Citation 'dietvorst2015algorithm' on page 7 undefined on input l
ine 110.


LaTeX Warning: Citation 'main2016cook' on page 7 undefined on input line 110.


Underfull \vbox (badness 1122) has occurred while \output is active [7.7]

LaTeX Warning: Citation 'alon2023human' on page 8 undefined on input line 124.


LaTeX Warning: Citation 'DBLP:journals/automatica/Bainbridge83' on page 8 undef
ined on input line 124.


LaTeX Warning: Citation 'ferguson2020high' on page 8 undefined on input line 12
4.


LaTeX Warning: Citation 'DBLP:conf/eaamo/Grgic-HlacaLWR22' on page 8 undefined 
on input line 125.


LaTeX Warning: Citation 'lee2018understanding' on page 8 undefined on input lin
e 125.


LaTeX Warning: Citation 'DBLP:conf/chi/0002HZ20' on page 8 undefined on input l
ine 126.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-1712-09124' on page 8 undefined
 on input line 126.


LaTeX Warning: Citation 'DBLP:conf/www/Grgic-HlacaRGW18' on page 8 undefined on
 input line 128.


Overfull \hbox (30.6207pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) place [[]] or fur-ther con-firm the stereo
-types [[],

Overfull \hbox (142.4989pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) agents tend to under-monitor when they per
-ceive affin-ity to-wards the mon-i-tor case at hand [[]],

Overfull \hbox (14.24838pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) or sim-ply when they deem their rea-son-in
g more ``hu-man'' than the ma-chine's [[]].

Overfull \hbox (38.19225pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) decision-making of the hu-man agents [[], 
[]].

LaTeX Warning: Citation 'englich2006playing' on page 8 undefined on input line 
132.


Overfull \hbox (2.2601pt too wide) in paragraph at lines 132--132
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 132--132
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

LaTeX Warning: Citation 'DBLP:journals/corr/abs-1812-03219' on page 8 undefined
 on input line 134.


LaTeX Warning: Citation 'albright2019if' on page 8 undefined on input line 134.



LaTeX Warning: Citation 'DBLP:journals/csur/GuidottiMRTGP19' on page 8 undefine
d on input line 140.


LaTeX Warning: Citation 'DBLP:conf/nips/LundbergL17' on page 8 undefined on inp
ut line 141.


LaTeX Warning: Citation 'DBLP:journals/expert/GuidottiMGPRT19' on page 8 undefi
ned on input line 141.


LaTeX Warning: Citation 'DBLP:conf/icml/KohL17' on page 8 undefined on input li
ne 141.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-2303-09297' on page 8 undefined
 on input line 141.


Overfull \hbox (80.86664pt too wide) in paragraph at lines 138--143
\T1/LinuxLibertineT-TLF/m/n/10 (-20) to fur-ther ex-plain the pre-dic-tions giv
en by a ma-chine. Ex-plain-able AI (XAI) [[]]
)

LaTeX Warning: Citation 'cortes2016l2r' on page 8 undefined on input line 273.

[8.8]

LaTeX Warning: Citation 'Chow1970' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'cortes2016l2r' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'Madras18' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'Mozannar20' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'Madras18' on page 9 undefined on input line 285.

(./L2R.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (9.70471pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dovremmo 

Overfull \hbox (9.31847pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigma 

Overfull \hbox (8.02188pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) vazionalei[]  

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (9.70471pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dovremmo 

Overfull \hbox (9.31847pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigma 

Overfull \hbox (8.02188pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) vazionalei[]  

LaTeX Warning: Citation 'Chow1970' on page 9 undefined on input line 3.


LaTeX Warning: Citation 'Chow1970' on page 9 undefined on input line 3.


LaTeX Warning: Citation 'ZhangSurv' on page 9 undefined on input line 6.


LaTeX Warning: Citation 'el_yaniv_foundation' on page 9 undefined on input line
 6.


LaTeX Warning: Citation 'HendrickxSurv' on page 9 undefined on input line 6.


LaTeX Warning: Citation 'HendrickxSurv' on page 9 undefined on input line 9.


LaTeX Warning: Citation 'HendrickxSurv' on page 9 undefined on input line 9.


LaTeX Warning: Citation 'ZhangSurv' on page 9 undefined on input line 9.


LaTeX Warning: Citation 'ZhangSurv' on page 9 undefined on input line 9.

[9.9]

LaTeX Warning: Citation 'GyorfiBayes' on page 10 undefined on input line 35.


LaTeX Warning: Citation 'outlier_survey_2004' on page 10 undefined on input lin
e 45.


LaTeX Warning: Citation 'anomaly_comprehensive_2020' on page 10 undefined on in
put line 45.


LaTeX Warning: Citation 'openset_surv' on page 10 undefined on input line 45.


Overfull \hbox (32.09886pt too wide) in paragraph at lines 45--46
\T1/LinuxLibertineT-TLF/m/it/10 (-20) tions\T1/LinuxLibertineT-TLF/m/n/10 (-20)
 . Most of the works in this par-tic-u-lar area frame the prob-lem as \T1/Linux
LibertineT-TLF/m/it/10 (-20) Out-lier de-tec-tion \T1/LinuxLibertineT-TLF/m/n/1
0 (-20) [[]]

LaTeX Warning: Citation 'Seo_Wallat_Graepel_Obermayer_2000' on page 10 undefine
d on input line 47.


LaTeX Warning: Citation 'Seo_Wallat_Graepel_Obermayer_2000' on page 10 undefine
d on input line 47.


LaTeX Warning: Citation 'Coles2001' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'Coles2001' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'Scheirer11' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'math11092171' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'ruddEVM' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'ruddEVM' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'vignotto_extreme_2020' on page 10 undefined on input l
ine 47.


Overfull \hbox (74.74547pt too wide) in paragraph at lines 47--48
\T1/LinuxLibertineT-TLF/m/n/10 (-20) cesses as a test-ing point to un-der-stand
 whether to re-ject a data point or not [[]].
[10.10]

LaTeX Warning: Citation 'Coenen2020ProbabilityOD' on page 11 undefined on input
 line 49.


LaTeX Warning: Citation 'Coenen2020ProbabilityOD' on page 11 undefined on input
 line 49.


LaTeX Warning: Citation 'Landgrebe' on page 11 undefined on input line 49.


LaTeX Warning: Citation 'fewshotanom' on page 11 undefined on input line 49.


LaTeX Warning: Citation 'AsifNets' on page 11 undefined on input line 51.


LaTeX Warning: Citation 'AsifNets' on page 11 undefined on input line 51.


LaTeX Warning: Citation 'Dalitz2009RejectOA' on page 11 undefined on input line
 55.


LaTeX Warning: Citation 'Grandvalet2008' on page 11 undefined on input line 55.



LaTeX Warning: Citation 'Jnior2017NearestND' on page 11 undefined on input line
 55.


LaTeX Warning: Citation 'hansen_error_reject_1997' on page 11 undefined on inpu
t line 62.


LaTeX Warning: Citation 'el_yaniv_foundation' on page 11 undefined on input lin
e 62.


Overfull \hbox (3.87013pt too wide) in paragraph at lines 60--66
\T1/LinuxLibertineT-TLF/m/n/10 (-20) tion $\OML/nxlmi/m/it/10 f$\T1/LinuxLibert
ineT-TLF/m/n/10 (-20) , and $\OML/nxlmi/m/it/10 ^^\$ \T1/LinuxLibertineT-TLF/m/
n/10 (-20) is the thresh-old hy-per-pa-ram-e-ter [[], []].

LaTeX Warning: Citation 'battisti_democracy' on page 11 undefined on input line
 68.


LaTeX Warning: Citation 'sousa_map' on page 11 undefined on input line 68.


Overfull \hbox (20.76775pt too wide) in paragraph at lines 68--69
\T1/LinuxLibertineT-TLF/m/n/10 (-20) sider the class-wise vari-ance of these pr
e-dic-tions as in-di-ca-tion of un-cer-tainty [[],

LaTeX Warning: Citation 'destefano_shakespear' on page 11 undefined on input li
ne 69.


LaTeX Warning: Citation 'brinkrolf_lvq' on page 11 undefined on input line 69.


LaTeX Warning: Citation 'tortorella_svm' on page 11 undefined on input line 73.



LaTeX Warning: Citation 'tortorella_svm' on page 11 undefined on input line 73.



LaTeX Warning: Citation 'Johannes_interpretable_conf' on page 11 undefined on i
nput line 74.

[11.11]

LaTeX Warning: Citation 'capitaine_frelicot' on page 12 undefined on input line
 76.


LaTeX Warning: Citation 'ceccotti_vajda' on page 12 undefined on input line 76.



LaTeX Warning: Citation 'Fischer_multiple_tau' on page 12 undefined on input li
ne 77.


LaTeX Warning: Citation 'pillai' on page 12 undefined on input line 77.


LaTeX Warning: Citation 'Fischer_variance' on page 12 undefined on input line 7
7.


Overfull \hbox (2.31824pt too wide) in paragraph at lines 76--78
\T1/LinuxLibertineT-TLF/m/n/10 (-20) [[], []]. Mul-ti-ple lo-cal thresh-olds $\
OML/nxlmi/m/it/10 ^^\[]; [] ; ^^\[]$ \T1/LinuxLibertineT-TLF/m/n/10 (-20) [[]]

LaTeX Warning: Citation 'HendrickxSurv' on page 12 undefined on input line 79.


LaTeX Warning: Citation 'cortes2016l2r' on page 12 undefined on input line 79.


LaTeX Warning: Citation 'Bartlett2008' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'RamaswamyReject' on page 12 undefined on input line 80
.


LaTeX Warning: Citation 'pugnana2023' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'pugnana2023' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'Ziyin2019' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'Grandvalet2008' on page 12 undefined on input line 81.



LaTeX Warning: Citation 'LIN2018' on page 12 undefined on input line 81.


LaTeX Warning: Citation 'Geifman2019SelectiveNetAD' on page 12 undefined on inp
ut line 81.


LaTeX Warning: Citation 'cortes2016l2r' on page 12 undefined on input line 86.


LaTeX Warning: Citation 'cortes2016l2r' on page 12 undefined on input line 86.

(/usr/share/texmf-dist/tex/latex/bbm-macros/ubbm.fd)

LaTeX Font Warning: Font shape `U/bbm/m/n' in size <5.5> not available
(Font)              size <5> substituted on input line 103.


LaTeX Warning: Citation 'Geifman2019SelectiveNetAD' on page 12 undefined on inp
ut line 109.

[12.12]

LaTeX Warning: Citation 'GeifmanNIPS17' on page 13 undefined on input line 111.



LaTeX Warning: Citation 'GeifmanNIPS17' on page 13 undefined on input line 111.



LaTeX Warning: Citation 'pmlr-v97-franc19a' on page 13 undefined on input line 
126.


LaTeX Warning: Citation 'JonesSKKL21' on page 13 undefined on input line 129.

) (./L2D.tex [13.13]

LaTeX Warning: Citation 'cortes2016l2r' on page 14 undefined on input line 75.


LaTeX Warning: Citation 'Madras18' on page 14 undefined on input line 77.


LaTeX Warning: Citation 'De2020Class' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Mozannar20' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Mozannar2023' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Okati2021' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Keswani2021' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Madras18' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Mozannar2023' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Martinez20' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Raghu2019TheAA' on page 14 undefined on input line 113
.


LaTeX Warning: Citation 'Verma2022Multi' on page 14 undefined on input line 128
.

[14.14]

LaTeX Warning: Citation 'Raghu2019TheAA' on page 15 undefined on input line 151
.


LaTeX Warning: Citation 'Raghu2019Med' on page 15 undefined on input line 152.


LaTeX Warning: Citation 'Bansal2021IsTM' on page 15 undefined on input line 156
.


LaTeX Warning: Citation 'Wilder2020' on page 15 undefined on input line 161.


LaTeX Warning: Citation 'Charusaie2022' on page 15 undefined on input line 164.



LaTeX Warning: Citation 'Charusaie2022' on page 15 undefined on input line 165.



LaTeX Warning: Citation 'Mozannar2023' on page 15 undefined on input line 173.


LaTeX Warning: Citation 'Mozannar2023' on page 15 undefined on input line 173.


Class acmart Warning: A possible image without description on input line 175.

[15.15]

LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 206.


LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 206.


LaTeX Warning: Citation 'Lin2004' on page 16 undefined on input line 210.


LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 211.


LaTeX Warning: Citation 'Charusaie2022' on page 16 undefined on input line 211.



LaTeX Warning: Citation 'Verma22' on page 16 undefined on input line 211.


LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 212.


LaTeX Warning: Citation 'Charusaie2022' on page 16 undefined on input line 217.


[16.16 <./media/joint_deferral_content_moderation.png>]

LaTeX Warning: Citation 'Liu2022' on page 17 undefined on input line 225.


LaTeX Warning: Citation 'Raman2021' on page 17 undefined on input line 226.


LaTeX Warning: Citation 'Dawid1982' on page 17 undefined on input line 229.


LaTeX Warning: Citation 'Verma22' on page 17 undefined on input line 229.


LaTeX Warning: Citation 'Verma22' on page 17 undefined on input line 229.


LaTeX Warning: Citation 'Bansal2021IsTM' on page 17 undefined on input line 234
.


LaTeX Warning: Citation 'Mozannar20' on page 17 undefined on input line 234.


LaTeX Warning: Citation 'Okati2021' on page 17 undefined on input line 234.


LaTeX Warning: Citation 'Raghu2019TheAA' on page 17 undefined on input line 234
.


LaTeX Warning: Citation 'Mozannar2023' on page 17 undefined on input line 237.


LaTeX Warning: Citation 'Madras18' on page 17 undefined on input line 249.


LaTeX Warning: Citation 'Mozannar20' on page 17 undefined on input line 249.


LaTeX Warning: Citation 'Pradier2021' on page 17 undefined on input line 250.


LaTeX Warning: Citation 'Madras18' on page 17 undefined on input line 250.

[17.17]

LaTeX Warning: Citation 'Wilder2020' on page 18 undefined on input line 255.


LaTeX Warning: Citation 'Mozannar2023' on page 18 undefined on input line 257.


LaTeX Warning: Citation 'Hemmer2022' on page 18 undefined on input line 285.


LaTeX Warning: Citation 'Verma2022Multi' on page 18 undefined on input line 287
.


LaTeX Warning: Citation 'Hemmer2022' on page 18 undefined on input line 289.


LaTeX Warning: Citation 'Gao2021' on page 18 undefined on input line 291.


LaTeX Warning: Citation 'Keswani2021' on page 18 undefined on input line 305.

[18.18]

LaTeX Warning: Citation 'Keswani2022' on page 19 undefined on input line 316.


LaTeX Warning: Citation 'Verma2022Multi' on page 19 undefined on input line 323
.


LaTeX Warning: Citation 'Shafer2008' on page 19 undefined on input line 323.


LaTeX Warning: Citation 'Angelopoulos2022' on page 19 undefined on input line 3
23.


LaTeX Warning: Citation 'Okati2021' on page 19 undefined on input line 329.


LaTeX Warning: Citation 'Mozannar2023' on page 19 undefined on input line 329.


LaTeX Warning: Citation 'De2020Class' on page 19 undefined on input line 331.


LaTeX Warning: Citation 'De2020Reg' on page 19 undefined on input line 331.


LaTeX Warning: Citation 'Leitao2022' on page 19 undefined on input line 342.


LaTeX Warning: Citation 'Hemmer2023' on page 19 undefined on input line 342.


LaTeX Warning: Citation 'Charusaie2022' on page 19 undefined on input line 344.



LaTeX Warning: Citation 'Cohn1994' on page 19 undefined on input line 344.

[19.19]

LaTeX Warning: Citation 'Hemmer2023' on page 20 undefined on input line 347.


LaTeX Warning: Citation 'Hemmer2023UserStudy' on page 20 undefined on input lin
e 359.


LaTeX Warning: Citation 'Papenmeier2023' on page 20 undefined on input line 362
.


LaTeX Warning: Citation 'Leitao2022' on page 20 undefined on input line 367.


LaTeX Warning: Citation 'Jones21' on page 20 undefined on input line 368.

[20.20]) (./human_interaction.tex

LaTeX Warning: Citation 'DBLP:journals/nn/VapnikV09' on page 21 undefined on in
put line 42.


LaTeX Warning: Citation 'DBLP:conf/kdd/BucilaCN06' on page 21 undefined on inpu
t line 42.


LaTeX Warning: Citation 'DBLP:journals/pieee/ZhuangQDXZZXH21' on page 21 undefi
ned on input line 42.


LaTeX Warning: Citation 'settles2009active' on page 21 undefined on input line 
42.


Overfull \hbox (43.57573pt too wide) in paragraph at lines 42--49
\T1/LinuxLibertineT-TLF/m/n/10 (-20) Trans-fer Learn-ing [[]], and Ac-tive Lear
n-ing [[]].

LaTeX Warning: Citation 'DBLP:journals/nn/VapnikV09' on page 21 undefined on in
put line 50.

[21.21]

LaTeX Warning: Citation 'DBLP:conf/kdd/BucilaCN06' on page 22 undefined on inpu
t line 70.


LaTeX Warning: Citation 'DBLP:journals/pieee/ZhuangQDXZZXH21' on page 22 undefi
ned on input line 93.


Overfull \hbox (149.376pt too wide) in paragraph at lines 93--97
\T1/LinuxLibertineT-TLF/m/n/10 (-20) tries to lever-age the knowl-edge of the T
eacher, and only then adapts it to the task at hand [[]].

LaTeX Warning: Citation 'settles2009active' on page 22 undefined on input line 
103.


LaTeX Warning: Citation 'settles2009active' on page 22 undefined on input line 
119.


LaTeX Warning: Citation 'DBLP:conf/nldb/MullerPBF22' on page 22 undefined on in
put line 119.


LaTeX Warning: Citation 'DBLP:journals/ml/CohnAL94' on page 22 undefined on inp
ut line 119.


LaTeX Warning: Citation 'DBLP:journals/ml/CohnAL94' on page 22 undefined on inp
ut line 120.

[22.22{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_kijugd.enc}]
[23.23]
Overfull \hbox (2.2601pt too wide) in paragraph at lines 214--214
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 214--214
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (5.42758pt too wide) in paragraph at lines 216--216
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) Abbiamo 

Overfull \hbox (1.56297pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) roberto 

Overfull \hbox (8.2248pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigmi 

Overfull \hbox (5.7366pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) rezionale 

Overfull \hbox (1.65099pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) sezione 

Overfull \hbox (14.38783pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) l'importanza 

Overfull \hbox (4.70122pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) fragilita', 

Overfull \hbox (5.42758pt too wide) in paragraph at lines 216--216
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) Abbiamo 

Overfull \hbox (1.56297pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) roberto 

Overfull \hbox (8.2248pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigmi 

Overfull \hbox (5.7366pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) rezionale 

Overfull \hbox (1.65099pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) sezione 

Overfull \hbox (14.38783pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) l'importanza 

Overfull \hbox (4.70122pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) fragilita', 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 217--217
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (5.5602pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) nell'altro 

Overfull \hbox (3.52669pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) munque 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 217--217
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (5.5602pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) nell'altro 

Overfull \hbox (3.52669pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) munque 

LaTeX Warning: Marginpar on page 24 moved.


LaTeX Warning: Marginpar on page 24 moved.


Underfull \hbox (badness 10000) in paragraph at lines 219--222


Overfull \hbox (2.2601pt too wide) in paragraph at lines 244--244
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.4399pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) mento? 

Overfull \hbox (5.03302pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) potrebbe 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 244--244
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.4399pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) mento? 

Overfull \hbox (5.03302pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) potrebbe 

LaTeX Warning: Marginpar on page 24 moved.


Underfull \hbox (badness 10000) in paragraph at lines 259--269

[24.24]

Class acmart Warning: A possible image without description on input line 297.


LaTeX Warning: Citation 'DBLP:conf/cvpr/JohnsonHMFZG17' on page 25 undefined on
 input line 299.


LaTeX Warning: Citation 'DBLP:conf/iui/GuoDAMCK22' on page 25 undefined on inpu
t line 304.


LaTeX Warning: Citation 'DBLP:conf/pldi/EllisWNSMHCST21' on page 25 undefined o
n input line 312.

[25.25]

LaTeX Warning: Citation 'DBLP:conf/emnlp/KassnerTSC21' on page 26 undefined on 
input line 336.


LaTeX Warning: Citation 'DBLP:conf/nips/LewisPPPKGKLYR020' on page 26 undefined
 on input line 336.


LaTeX Warning: Citation 'DBLP:conf/ijcai/ClarkTR20' on page 26 undefined on inp
ut line 336.


Overfull \hbox (35.3791pt too wide) in paragraph at lines 336--343
\T1/LinuxLibertineT-TLF/m/n/10 (-20) builds on top of two other fam-i-lies, kno
wl-edge in-jec-tion mod-els [[]]

LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 380.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 380.


Class acmart Warning: A possible image without description on input line 382.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 384.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 390.


LaTeX Warning: Citation 'DBLP:conf/emnlp/BostromZCD21' on page 26 undefined on 
input line 392.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MurtyMLR22' on page 26 undefined on in
put line 393.


LaTeX Warning: Citation 'DBLP:conf/nips/LewisPPPKGKLYR020' on page 26 undefined
 on input line 404.


LaTeX Warning: Citation 'DBLP:conf/aaai/HwangBBDSBC21' on page 26 undefined on 
input line 406.


LaTeX Warning: Citation 'DBLP:journals/cacm/VrandecicK14' on page 26 undefined 
on input line 406.


LaTeX Warning: Citation 'wang2017fvqa' on page 26 undefined on input line 431.

[26.26 <./media/clever.pdf>]

LaTeX Warning: Citation 'MalandriMMN23' on page 27 undefined on input line 457.



LaTeX Warning: Citation 'DBLP:journals/aim/AmershiCKK14' on page 27 undefined o
n input line 463.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 27 undefined on input 
line 463.

[27.27]
Overfull \hbox (2.2601pt too wide) in paragraph at lines 489--489
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.90285pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) lascerei 

Overfull \hbox (3.19742pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tostante 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 489--489
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.90285pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) lascerei 

Overfull \hbox (3.19742pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tostante 

LaTeX Warning: Citation 'DBLP:conf/ijcai/RossHD17' on page 28 undefined on inpu
t line 493.


LaTeX Warning: Citation 'teso2019toward' on page 28 undefined on input line 493
.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 28 undefined on input 
line 493.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 28 undefined on input 
line 504.


LaTeX Warning: Citation 'DBLP:conf/kdd/WangKNSNCVV022' on page 28 undefined on 
input line 506.

[28.28 <./media/hydrant_only.png>]

LaTeX Warning: Citation 'Popordanoska2020' on page 29 undefined on input line 5
12.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-2012-02898' on page 29 undefine
d on input line 514.


Overfull \hbox (40.68759pt too wide) in paragraph at lines 511--515
\T1/LinuxLibertineT-TLF/m/n/10 (-20) the cor-rec-tion is again an added com-po-
nent of the ma-chine ob-jec-tive [[]]. 

LaTeX Warning: Citation 'DBLP:journals/datamine/BontempelliGPT22' on page 29 un
defined on input line 517.

[29.29])
Overfull \hbox (9.70557pt too wide) in paragraph at lines 305--305
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) richiamare 

Overfull \hbox (9.70557pt too wide) in paragraph at lines 305--305
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) richiamare 

LaTeX Warning: Citation 'Sarkar2023' on page 30 undefined on input line 312.

[30.30] (./conclusions.tex)

LaTeX Warning: Empty bibliography on input line 338.

[31.31] (./appendices.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (6.47256pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tosezione 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (6.47256pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tosezione 

LaTeX Warning: Citation 'Fisher1922' on page 32 undefined on input line 7.


LaTeX Warning: Citation 'Lin2004' on page 32 undefined on input line 8.


LaTeX Warning: Citation 'Bartlett2006' on page 32 undefined on input line 8.


LaTeX Warning: Citation 'Long2013' on page 32 undefined on input line 12.


LaTeX Warning: Citation 'Mozannar2023' on page 32 undefined on input line 14.


LaTeX Warning: Citation 'Verma22' on page 32 undefined on input line 14.


LaTeX Warning: Citation 'Lin2004' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Liu2007' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Tewari2007' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Zou2008' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Mozannar20' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Verma22' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Fisher1922' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Gerow1989' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Bartlett2006' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Lin2004' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Neykov2016' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Steinwart2007' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Tewari2007' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Bartlett2006' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Dawid1982' on page 32 undefined on input line 22.


LaTeX Warning: Citation 'Verma22' on page 32 undefined on input line 22.


LaTeX Warning: Citation 'Vaicenavicius2019' on page 32 undefined on input line 
22.


LaTeX Warning: Citation 'SilvaFilho2023' on page 32 undefined on input line 25.



LaTeX Warning: Citation 'Vaicenavicius2019' on page 32 undefined on input line 
29.


LaTeX Warning: Citation 'Kull2019' on page 32 undefined on input line 30.


LaTeX Warning: Citation 'SilvaFilho2023' on page 32 undefined on input line 30.


[32.32]

LaTeX Warning: Citation 'Verma2022Multi' on page 33 undefined on input line 32.



LaTeX Warning: Citation 'Verma22' on page 33 undefined on input line 32.


LaTeX Warning: Citation 'Verma22' on page 33 undefined on input line 40.


LaTeX Warning: Citation 'Verma2022Multi' on page 33 undefined on input line 40.



LaTeX Warning: Citation 'Long2013' on page 33 undefined on input line 46.


LaTeX Warning: Citation 'Long2013' on page 33 undefined on input line 46.


LaTeX Warning: Citation 'cortes2016l2r' on page 33 undefined on input line 47.


LaTeX Warning: Citation 'Mozannar20' on page 33 undefined on input line 47.


LaTeX Warning: Citation 'Mozannar2023' on page 33 undefined on input line 47.


LaTeX Warning: Citation 'cortes2016l2r' on page 33 undefined on input line 50.


LaTeX Warning: Citation 'Mozannar2023' on page 33 undefined on input line 50.


LaTeX Warning: Citation 'Mozannar20' on page 33 undefined on input line 50.


LaTeX Warning: Citation 'Mozannar2023' on page 33 undefined on input line 64.

[33.33] [34.34]
Overfull \hbox (10.90298pt too wide) in paragraph at lines 92--92
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Architecture| 

Overfull \hbox (5.88702pt too wide) in paragraph at lines 92--92
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Theoretical

Underfull \hbox (badness 10000) in paragraph at lines 92--92
\T1/LinuxLibertineT-TLF/m/n/10 (+20) guar-an-

Overfull \hbox (26.71838pt too wide) in paragraph at lines 92--92
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Constraints| 

LaTeX Warning: Citation 'Raghu2019TheAA' on page 35 undefined on input line 93.



Overfull \hbox (2.99666pt too wide) in paragraph at lines 93--93
[]|[]| 

Overfull \hbox (8.51001pt too wide) in paragraph at lines 93--93
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Budget| 

Underfull \hbox (badness 10000) in paragraph at lines 93--93
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Retinal

Underfull \hbox (badness 10000) in paragraph at lines 93--93
\T1/LinuxLibertineT-TLF/m/n/10 (+20) fun-dus

Underfull \hbox (badness 10000) in paragraph at lines 93--93
\T1/LinuxLibertineT-TLF/m/n/10 (+20) pho-

LaTeX Warning: Citation 'Wilder2020' on page 35 undefined on input line 94.


Underfull \hbox (badness 10000) in paragraph at lines 94--94
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Staged,

Underfull \hbox (badness 10000) in paragraph at lines 94--94
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 94--94
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy

Underfull \hbox (badness 10000) in paragraph at lines 94--94
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Zoo,

Underfull \hbox (badness 10000) in paragraph at lines 94--94
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Breast

LaTeX Warning: Citation 'Bansal2021IsTM' on page 35 undefined on input line 95.



Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) man

Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) credit,

Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) FICO,

Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Com-pas,

LaTeX Warning: Citation 'Madras18' on page 35 undefined on input line 96.


Underfull \hbox (badness 10000) in paragraph at lines 96--96
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Joint

Overfull \hbox (14.13278pt too wide) in paragraph at lines 96--96
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Fairness,

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Cov-

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) er-

Underfull \hbox (badness 10000) in paragraph at lines 96--96
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Com-pas,

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Her-itage

LaTeX Warning: Citation 'Mozannar20' on page 35 undefined on input line 97.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 97--97
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) , CI-

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) FAR10H,

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CheX-

Overfull \hbox (22.41237pt too wide) in paragraph at lines 97--98
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/clinicalml/learn-

LaTeX Warning: Citation 'Verma22' on page 35 undefined on input line 98.


Overfull \hbox (8.51001pt too wide) in paragraph at lines 98--98
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Budget| 

Underfull \hbox (badness 10000) in paragraph at lines 98--98
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 10,

Overfull \hbox (6.44347pt too wide) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (-20) HAM10000,

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy-

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Zoo,

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate-

Overfull \hbox (5.80733pt too wide) in paragraph at lines 98--99
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/rajevv/OvA-

LaTeX Warning: Citation 'Charusaie2022' on page 35 undefined on input line 99.


Underfull \hbox (badness 10000) in paragraph at lines 99--99
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Lim-ited

Underfull \hbox (badness 10000) in paragraph at lines 99--99
\T1/LinuxLibertineT-TLF/m/n/10 (+20) hu-man

Underfull \hbox (badness 10000) in paragraph at lines 99--99
\T1/LinuxLibertineT-TLF/m/n/10 (+20) pre-dic-

Underfull \hbox (badness 10000) in paragraph at lines 99--99
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Overfull \hbox (87.11462pt too wide) in paragraph at lines 99--100
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/clinicalml/active_le
arn_to_defer| 

LaTeX Warning: Citation 'Liu2022' on page 35 undefined on input line 100.


Underfull \hbox (badness 10000) in paragraph at lines 100--100
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 100--100
\T1/LinuxLibertineT-TLF/m/n/10 (+20) MIMIC-

Underfull \hbox (badness 10000) in paragraph at lines 100--100
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Her-itage,

Underfull \hbox (badness 10000) in paragraph at lines 100--100
\T1/LinuxLibertineT-TLF/m/n/10 (+20) MIMIC-

Underfull \hbox (badness 10000) in paragraph at lines 100--101
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) https://github.com/liu-

Underfull \hbox (badness 10000) in paragraph at lines 100--101
\T1/LinuxLibertineT-TLF/m/n/10 (+20) res/Learning-to-Defer-with-

LaTeX Warning: Citation 'Raman2021' on page 35 undefined on input line 101.


Underfull \hbox (badness 10000) in paragraph at lines 101--101
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Synthetic

Underfull \hbox (badness 10000) in paragraph at lines 101--101
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

LaTeX Warning: Citation 'Pradier2021' on page 35 undefined on input line 102.


Underfull \hbox (badness 10000) in paragraph at lines 102--102
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Joint

Overfull \hbox (12.5326pt too wide) in paragraph at lines 102--102
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Sparsity

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) of

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) the

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) de-

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) fer-

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) ral

LaTeX Warning: Citation 'Mozannar2023' on page 35 undefined on input line 103.


Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Lim-ited

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) hu-man

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) pre-dic-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) tions,

Overfull \hbox (14.13278pt too wide) in paragraph at lines 103--103
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Fairness,

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Cov-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) er-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 10H,

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Speach,

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Com-pas,

Overfull \hbox (5.06406pt too wide) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (-20) ChestXRay| 

Overfull \hbox (76.16968pt too wide) in paragraph at lines 103--104
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/clinicalml/human_ai_
deferral| 

LaTeX Warning: Citation 'Okati2021' on page 35 undefined on input line 104.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 104--104
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 104--104
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 104--104
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy-

Underfull \hbox (badness 10000) in paragraph at lines 104--105
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-11) https://github.com/Networks-

Underfull \hbox (badness 10000) in paragraph at lines 104--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Learning/differentiable-

LaTeX Warning: Citation 'De2020Class' on page 35 undefined on input line 105.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 105--105
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 105--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 105--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Stare,

Underfull \hbox (badness 10000) in paragraph at lines 105--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Mes-si-dor,

Underfull \hbox (badness 10000) in paragraph at lines 105--106
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-11) https://github.com/Networks-

Underfull \hbox (badness 10000) in paragraph at lines 105--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Learning/classification-

LaTeX Warning: Citation 'De2020Reg' on page 35 undefined on input line 106.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 106--106
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Speech,

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Stare-H,

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Stare-D,

Underfull \hbox (badness 10000) in paragraph at lines 106--107
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-11) https://github.com/Networks-

Underfull \hbox (badness 10000) in paragraph at lines 106--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Learning/regression-under-

LaTeX Warning: Citation 'Hemmer2023' on page 35 undefined on input line 107.


Underfull \hbox (badness 10000) in paragraph at lines 107--107
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Limited

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hu-man

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Pre-dic-

Underfull \hbox (badness 10000) in paragraph at lines 107--107
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 100,

Overfull \hbox (5.06406pt too wide) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (-20) ChestXRay| 

Overfull \hbox (41.64806pt too wide) in paragraph at lines 107--108
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/ptrckhmmr/learning-

Underfull \hbox (badness 10000) in paragraph at lines 107--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) to-deferwith-limited-expert-

LaTeX Warning: Citation 'Hemmer2022' on page 35 undefined on input line 108.


Underfull \hbox (badness 10000) in paragraph at lines 108--108
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Speech,

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 100,

Overfull \hbox (5.06406pt too wide) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (-20) ChestXRay| 

Overfull \hbox (36.38547pt too wide) in paragraph at lines 108--109
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/ptrckhmmr/human-

LaTeX Warning: Citation 'Verma2022Multi' on page 35 undefined on input line 109
.


Underfull \hbox (badness 4846) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) of J,

Underfull \hbox (badness 10000) in paragraph at lines 109--109
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Overfull \hbox (6.44347pt too wide) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (-20) HAM10000,

Underfull \hbox (badness 10000) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy-

Underfull \hbox (badness 10000) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Zoo,

Underfull \hbox (badness 10000) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate-

Overfull \hbox (29.51352pt too wide) in paragraph at lines 109--110
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/rajevv/Multi_L2D| 

LaTeX Warning: Citation 'Gao2021' on page 35 undefined on input line 110.


Underfull \hbox (badness 10000) in paragraph at lines 110--110
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Staged,

Underfull \hbox (badness 10000) in paragraph at lines 110--110
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 110--110
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Scene,

Underfull \hbox (badness 10000) in paragraph at lines 110--110
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Yeast,

Underfull \hbox (badness 10000) in paragraph at lines 110--110
\T1/LinuxLibertineT-TLF/m/n/10 (+20) MLC,

Overfull \hbox (16.05214pt too wide) in paragraph at lines 110--111
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/ruijiang81/hai-

LaTeX Warning: Citation 'Keswani2021' on page 35 undefined on input line 111.


Overfull \hbox (14.13278pt too wide) in paragraph at lines 111--111
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Fairness,

Overfull \hbox (6.3736pt too wide) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (-20) Sparse

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) com-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) mit-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) tee,

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hu-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) man

Overfull \hbox (13.12315pt too wide) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (-20) dropout,

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hu-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) man

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate

Overfull \hbox (48.74487pt too wide) in paragraph at lines 111--112
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/vijaykeswani/Deferra
l-

LaTeX Warning: Citation 'Keswani2022' on page 35 undefined on input line 112.


Underfull \hbox (badness 10000) in paragraph at lines 112--112
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Joint,

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Lim-ited

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) ground

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Twit-ter

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Eng-lish

Overfull \hbox (42.84532pt too wide) in paragraph at lines 112--113
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/vijaykeswani/Online-

[35.35] [36.36] [37.37] [38.38]
(/usr/share/texmf-dist/tex/generic/stringenc/se-pdfdoc.def)
(/usr/share/texmf-dist/tex/generic/stringenc/se-utf8.def) [39.39])

LaTeX Warning: Empty bibliography on input line 348.


Class acmart Warning: Some images may lack descriptions.

(./main.aux (./appendices.aux))

LaTeX Font Warning: Size substitutions with differences
(Font)              up to 0.5pt have occurred.


LaTeX Warning: There were undefined references.


Package biblatex Warning: Please (re)run Biber on the file:
(biblatex)                main
(biblatex)                and rerun LaTeX afterwards.

 )
(see the transcript file for additional information) </home/aslan/.texlive/texm
f-var/fonts/pk/ljfour/public/bbm/bbm10.600pk></usr/share/texmf-dist/fonts/type1
/public/newtx/LibertineMathMI.pfb></usr/share/texmf-dist/fonts/type1/public/new
tx/LibertineMathMI5.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/Liberti
neMathMI7.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/LibertineMathRM.p
fb></usr/share/texmf-dist/fonts/type1/public/libertine/LinBiolinumT.pfb></usr/s
hare/texmf-dist/fonts/type1/public/libertine/LinBiolinumTB.pfb></usr/share/texm
f-dist/fonts/type1/public/libertine/LinBiolinumTI.pfb></usr/share/texmf-dist/fo
nts/type1/public/libertine/LinLibertineT.pfb></usr/share/texmf-dist/fonts/type1
/public/libertine/LinLibertineTB.pfb></usr/share/texmf-dist/fonts/type1/public/
libertine/LinLibertineTBI.pfb></usr/share/texmf-dist/fonts/type1/public/liberti
ne/LinLibertineTI.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/NewTXMI.p
fb></usr/share/texmf-dist/fonts/type1/public/newtx/NewTXMI7.pfb></usr/share/tex
mf-dist/fonts/type1/public/newtx/stxscr.pfb></usr/share/texmf-dist/fonts/type1/
public/newtx/txexas.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/txexs.p
fb></usr/share/texmf-dist/fonts/type1/public/newtx/txmiaX.pfb></usr/share/texmf
-dist/fonts/type1/public/txfonts/txsyb.pfb></usr/share/texmf-dist/fonts/type1/p
ublic/txfonts/txsyc.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/txsys.p
fb>
Output written on main.pdf (39 pages, 2846366 bytes).
Transcript written on main.log.
This is pdfTeX, Version 3.141592653-2.6-1.40.25 (TeX Live 2023/Arch Linux) (preloaded format=pdflatex)
 restricted \write18 enabled.
entering extended mode
(./main.tex
LaTeX2e <2022-11-01> patch level 1
L3 programming layer <2023-02-22> (./acmart.cls
Document Class: acmart 2022/10/24 v1.88 Typesetting articles for the Associatio
n for Computing Machinery
(/usr/share/texmf-dist/tex/latex/xkeyval/xkeyval.sty
(/usr/share/texmf-dist/tex/generic/xkeyval/xkeyval.tex
(/usr/share/texmf-dist/tex/generic/xkeyval/xkvutils.tex
(/usr/share/texmf-dist/tex/generic/xkeyval/keyval.tex))))
(/usr/share/texmf-dist/tex/generic/xstring/xstring.sty
(/usr/share/texmf-dist/tex/generic/xstring/xstring.tex))
(/usr/share/texmf-dist/tex/generic/iftex/iftex.sty)
(/usr/share/texmf-dist/tex/latex/amscls/amsart.cls
Document Class: amsart 2020/05/29 v2.20.6
(/usr/share/texmf-dist/tex/latex/amsmath/amsmath.sty
For additional information on amsmath, use the `?' option.
(/usr/share/texmf-dist/tex/latex/amsmath/amstext.sty
(/usr/share/texmf-dist/tex/latex/amsmath/amsgen.sty))
(/usr/share/texmf-dist/tex/latex/amsmath/amsbsy.sty)
(/usr/share/texmf-dist/tex/latex/amsmath/amsopn.sty))
(/usr/share/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf-dist/tex/latex/amsfonts/amsfonts.sty))
(/usr/share/texmf-dist/tex/latex/microtype/microtype.sty
(/usr/share/texmf-dist/tex/latex/etoolbox/etoolbox.sty)
(/usr/share/texmf-dist/tex/latex/microtype/microtype-pdftex.def)
(/usr/share/texmf-dist/tex/latex/microtype/microtype.cfg))
(/usr/share/texmf-dist/tex/latex/booktabs/booktabs.sty)
(/usr/share/texmf-dist/tex/latex/refcount/refcount.sty
(/usr/share/texmf-dist/tex/generic/ltxcmds/ltxcmds.sty)
(/usr/share/texmf-dist/tex/generic/infwarerr/infwarerr.sty))
(/usr/share/texmf-dist/tex/latex/totpages/totpages.sty
(/usr/share/texmf-dist/tex/latex/everyshi/everyshi.sty))
(/usr/share/texmf-dist/tex/latex/environ/environ.sty
(/usr/share/texmf-dist/tex/latex/trimspaces/trimspaces.sty))
(/usr/share/texmf-dist/tex/latex/textcase/textcase.sty)
(/usr/share/texmf-dist/tex/latex/hyperxmp/hyperxmp.sty
(/usr/share/texmf-dist/tex/latex/kvoptions/kvoptions.sty
(/usr/share/texmf-dist/tex/latex/kvsetkeys/kvsetkeys.sty))
(/usr/share/texmf-dist/tex/generic/pdfescape/pdfescape.sty
(/usr/share/texmf-dist/tex/generic/pdftexcmds/pdftexcmds.sty))
(/usr/share/texmf-dist/tex/generic/stringenc/stringenc.sty)
(/usr/share/texmf-dist/tex/generic/intcalc/intcalc.sty)
(/usr/share/texmf-dist/tex/latex/ifmtarg/ifmtarg.sty)
(/usr/share/texmf-dist/tex/latex/base/ifthen.sty)
(/usr/share/texmf-dist/tex/latex/oberdiek/ifdraft.sty)
(/usr/share/texmf-dist/tex/generic/iftex/ifluatex.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/hyperref.sty
(/usr/share/texmf-dist/tex/generic/kvdefinekeys/kvdefinekeys.sty)
(/usr/share/texmf-dist/tex/latex/hycolor/hycolor.sty)
(/usr/share/texmf-dist/tex/latex/letltxmacro/letltxmacro.sty)
(/usr/share/texmf-dist/tex/latex/auxhook/auxhook.sty)
(/usr/share/texmf-dist/tex/latex/hyperref/nameref.sty
(/usr/share/texmf-dist/tex/generic/gettitlestring/gettitlestring.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/pd1enc.def)
(/usr/share/texmf-dist/tex/generic/etexcmds/etexcmds.sty)
(/usr/share/texmf-dist/tex/latex/hyperref/puenc.def)
(/usr/share/texmf-dist/tex/latex/url/url.sty)
(/usr/share/texmf-dist/tex/generic/bitset/bitset.sty
(/usr/share/texmf-dist/tex/generic/bigintcalc/bigintcalc.sty))
(/usr/share/texmf-dist/tex/latex/base/atbegshi-ltx.sty))
(/usr/share/texmf-dist/tex/latex/hyperref/hpdftex.def
(/usr/share/texmf-dist/tex/latex/base/atveryend-ltx.sty)
(/usr/share/texmf-dist/tex/latex/rerunfilecheck/rerunfilecheck.sty
(/usr/share/texmf-dist/tex/generic/uniquecounter/uniquecounter.sty)))
(/usr/share/texmf-dist/tex/latex/graphics/graphicx.sty
(/usr/share/texmf-dist/tex/latex/graphics/graphics.sty
(/usr/share/texmf-dist/tex/latex/graphics/trig.sty)
(/usr/share/texmf-dist/tex/latex/graphics-cfg/graphics.cfg)
(/usr/share/texmf-dist/tex/latex/graphics-def/pdftex.def)))
(/usr/share/texmf-dist/tex/latex/xcolor/xcolor.sty
(/usr/share/texmf-dist/tex/latex/graphics-cfg/color.cfg)
(/usr/share/texmf-dist/tex/latex/graphics/mathcolor.ltx))
(/usr/share/texmf-dist/tex/latex/geometry/geometry.sty
(/usr/share/texmf-dist/tex/generic/iftex/ifvtex.sty))
(/usr/share/texmf-dist/tex/latex/ncctools/manyfoot.sty
(/usr/share/texmf-dist/tex/latex/ncctools/nccfoots.sty))
(/usr/share/texmf-dist/tex/generic/pdftex/glyphtounicode.tex)
(/usr/share/texmf-dist/tex/latex/cmap/cmap.sty)
(/usr/share/texmf-dist/tex/latex/base/fontenc.sty<<t1.cmap>>)
(/usr/share/texmf-dist/tex/latex/libertine/libertine.sty
(/usr/share/texmf-dist/tex/generic/iftex/ifxetex.sty)
(/usr/share/texmf-dist/tex/latex/base/textcomp.sty)
(/usr/share/texmf-dist/tex/latex/base/fontenc.sty)
(/usr/share/texmf-dist/tex/latex/fontaxes/fontaxes.sty)
(/usr/share/texmf-dist/tex/latex/libertine/LinLibertine_I.tex))
(/usr/share/texmf-dist/tex/latex/inconsolata/zi4.sty
`inconsolata-zi4' v1.12, 2019/05/17 Text macros for Inconsolata (msharpe))
(/usr/share/texmf-dist/tex/latex/newtx/newtxmath.sty
`newtxmath' v1.71, 2022/01/16 Math macros based originally on txfonts (msharpe)
(/usr/share/texmf-dist/tex/latex/oberdiek/centernot.sty)
(/usr/share/texmf-dist/tex/generic/kastrup/binhex.tex)
amsthm NOT loaded
) (/usr/share/texmf-dist/tex/latex/caption/caption.sty
(/usr/share/texmf-dist/tex/latex/caption/caption3.sty
(/usr/share/texmf-dist/tex/latex/caption/caption-ams-smf.sto)))
(/usr/share/texmf-dist/tex/latex/float/float.sty)
(/usr/share/texmf-dist/tex/latex/comment/comment.sty
Excluding comment 'comment') Excluding comment 'CCSXML'
(/usr/share/texmf-dist/tex/latex/fancyhdr/fancyhdr.sty) Special comment 'acks'
(/usr/share/texmf-dist/tex/latex/libertine/T1LinuxLibertineT-TLF.fd))
(/usr/share/texmf-dist/tex/latex/xargs/xargs.sty)
(/usr/share/texmf-dist/tex/latex/bbm-macros/bbm.sty)
(/usr/share/texmf-dist/tex/latex/optidef/optidef.sty
(/usr/share/texmf-dist/tex/latex/mathtools/mathtools.sty
(/usr/share/texmf-dist/tex/latex/tools/calc.sty)
(/usr/share/texmf-dist/tex/latex/mathtools/mhsetup.sty))
(/usr/share/texmf-dist/tex/latex/xifthen/xifthen.sty)
(/usr/share/texmf-dist/tex/latex/l3packages/xparse/xparse.sty
(/usr/share/texmf-dist/tex/latex/l3kernel/expl3.sty
(/usr/share/texmf-dist/tex/latex/l3backend/l3backend-pdftex.def))))
(/usr/share/texmf-dist/tex/latex/enumitem/enumitem.sty)
(/usr/share/texmf-dist/tex/latex/graphics/lscape.sty)
(/usr/share/texmf-dist/tex/latex/tools/longtable.sty)
(/usr/share/texmf-dist/tex/latex/todonotes/todonotes.sty
(/usr/share/texmf-dist/tex/latex/pgf/frontendlayer/tikz.sty
(/usr/share/texmf-dist/tex/latex/pgf/basiclayer/pgf.sty
(/usr/share/texmf-dist/tex/latex/pgf/utilities/pgfrcs.sty
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfutil-common.tex)
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfutil-latex.def)
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfrcs.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/pgf.revision.tex)))
(/usr/share/texmf-dist/tex/latex/pgf/basiclayer/pgfcore.sty
(/usr/share/texmf-dist/tex/latex/pgf/systemlayer/pgfsys.sty
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsys.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfkeyslibraryfiltered.code.te
x)) (/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgf.cfg)
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-pdftex.def
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsys-common-pdf.def)))
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsyssoftpath.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/systemlayer/pgfsysprotocol.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcore.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathutil.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathparser.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.basic.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.trigonometric.code
.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.random.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.comparison.code.te
x) (/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.base.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.round.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.misc.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfunctions.integerarithmetics
.code.tex) (/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathcalc.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmathfloat.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfint.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepoints.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathconstruct.code.tex
) (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathusage.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorescopes.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoregraphicstate.code.tex)

(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransformations.code.t
ex) (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorequick.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreobjects.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepathprocessing.code.te
x) (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorearrows.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreshade.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreimage.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoreexternal.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorelayers.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcoretransparency.code.tex)
 (/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorepatterns.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/basiclayer/pgfcorerdf.code.tex)))
(/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmoduleshapes.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmoduleplot.code.tex)
(/usr/share/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-0-65.sty)
(/usr/share/texmf-dist/tex/latex/pgf/compatibility/pgfcomp-version-1-18.sty))
(/usr/share/texmf-dist/tex/latex/pgf/utilities/pgffor.sty
(/usr/share/texmf-dist/tex/latex/pgf/utilities/pgfkeys.sty
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgfkeys.code.tex))
(/usr/share/texmf-dist/tex/latex/pgf/math/pgfmath.sty
(/usr/share/texmf-dist/tex/generic/pgf/math/pgfmath.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/utilities/pgffor.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/tikz.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/pgflibraryplothandlers.code.te
x) (/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmodulematrix.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
topaths.code.tex)))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
positioning.code.tex)) (/usr/share/texmf-dist/tex/latex/doublestroke/dsfont.sty
) (/usr/share/texmf-dist/tex/latex/makecell/makecell.sty
(/usr/share/texmf-dist/tex/latex/tools/array.sty))
(/usr/share/texmf-dist/tex/latex/multirow/multirow.sty)
(/usr/share/texmf-dist/tex/latex/graphics/rotating.sty)
(/usr/share/texmf-dist/tex/latex/caption/subcaption.sty)
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
arrows.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/pgflibraryarrows.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.geometric.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.geomet
ric.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.misc.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.misc.c
ode.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.symbols.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.symbol
s.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.arrows.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.arrows
.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.callouts.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.callou
ts.code.tex))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
shapes.multipart.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/libraries/shapes/pgflibraryshapes.multip
art.code.tex)))
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
calc.code.tex)
(/usr/share/texmf-dist/tex/generic/pgf/frontendlayer/tikz/libraries/tikzlibrary
decorations.code.tex
(/usr/share/texmf-dist/tex/generic/pgf/modules/pgfmoduledecorations.code.tex))
(/usr/share/texmf-dist/tex/latex/varwidth/varwidth.sty)
(/usr/share/texmf-dist/tex/latex/biblatex/biblatex.sty
(/usr/share/texmf-dist/tex/latex/logreq/logreq.sty
(/usr/share/texmf-dist/tex/latex/logreq/logreq.def))
(/usr/share/texmf-dist/tex/latex/biblatex/blx-dm.def)
(/usr/share/texmf-dist/tex/latex/biblatex/blx-compat.def)
(/usr/share/texmf-dist/tex/latex/biblatex/biblatex.def)
(/usr/share/texmf-dist/tex/latex/biblatex/blx-natbib.def) (./acmnumeric.bbx
(/usr/share/texmf-dist/tex/latex/biblatex-trad/trad-plain.bbx
(/usr/share/texmf-dist/tex/latex/biblatex-trad/trad-standard.bbx
(/usr/share/texmf-dist/tex/latex/biblatex/bbx/standard.bbx)))
(/usr/share/texmf-dist/tex/latex/biblatex-software/software.bbx
(/usr/share/texmf-dist/tex/latex/xurl/xurl.sty
xurl: Set penalties for biblatex
))) (./acmnumeric.cbx (/usr/share/texmf-dist/tex/latex/biblatex/cbx/numeric.cbx
)) (/usr/share/texmf-dist/tex/latex/biblatex/biblatex.cfg)
(/usr/share/texmf-dist/tex/latex/biblatex/blx-case-expl3.sty))
Excluding comment 'screenonly' Include comment 'printonly'
Include comment 'anonsuppress'

LaTeX Warning: Unused global option(s):
    [natbib=false].

(./main.aux (./appendices.aux))
(/usr/share/texmf-dist/tex/latex/newtx/omlnxlmi.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxexa.fd)
(/usr/share/texmf-dist/tex/latex/newtx/lmsntxsy.fd)
(/usr/share/texmf-dist/tex/latex/newtx/lmxntxexx.fd)
(/usr/share/texmf-dist/tex/latex/libertine/OT1LinuxLibertineT-TLF.fd)<<ot1.cmap
>><<oml.cmap>> (/usr/share/texmf-dist/tex/latex/amsfonts/umsa.fd)
(/usr/share/texmf-dist/tex/latex/amsfonts/umsb.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxmia.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxsym.fd)
(/usr/share/texmf-dist/tex/latex/newtx/untxsyc.fd) (./main.out) (./main.out)
(/usr/share/texmf-dist/tex/context/base/mkii/supp-pdf.mkii
[Loading MPS to PDF converter (version 2006.09.02).]
) (/usr/share/texmf-dist/tex/latex/epstopdf-pkg/epstopdf-base.sty
(/usr/share/texmf-dist/tex/latex/latexconfig/epstopdf-sys.cfg))
*geometry* driver: auto-detecting
*geometry* detected driver: pdftex
(/usr/share/texmf-dist/tex/latex/upquote/upquote.sty)
(/usr/share/texmf-dist/tex/latex/caption/ltcaption.sty)

Package todonotes Warning: The length marginparwidth is less than 2cm and will 
most likely cause issues with the appearance of inserted todonotes. The issue c
an be solved by adding a line like \setlength {\marginparwidth }{2cm} prior to 
loading the todonotes package. on input line 144.

(/usr/share/texmf-dist/tex/latex/biblatex/lbx/american.lbx
(/usr/share/texmf-dist/tex/latex/biblatex-software/english-software.lbx
(/usr/share/texmf-dist/tex/latex/biblatex/lbx/english.lbx))
(/usr/share/texmf-dist/tex/latex/biblatex-software/english-software.lbx
(/usr/share/texmf-dist/tex/latex/biblatex/lbx/english.lbx))) (./main.bbl)
Excluding 'CCSXML' comment.
(/usr/share/texmf-dist/tex/latex/libertine/T1LinuxBiolinumT-TLF.fd)
(/usr/share/texmf-dist/tex/latex/libertine/TS1LinuxLibertineT-TLF.fd)
(/usr/share/texmf-dist/tex/latex/microtype/mt-msa.cfg)
(/usr/share/texmf-dist/tex/latex/microtype/mt-msb.cfg) (./introduction.tex

LaTeX Warning: Citation 'dietvorst2015algorithm' on page 1 undefined on input l
ine 16.


LaTeX Warning: Citation 'lee2004trust' on page 1 undefined on input line 16.


LaTeX Warning: Citation 'dietvorst2015algorithm' on page 1 undefined on input l
ine 18.


LaTeX Warning: Citation 'logg2019algorithm' on page 1 undefined on input line 1
8.


Overfull \hbox (2.52794pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) assisted 

Overfull \hbox (5.77692pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Decision- 

Overfull \hbox (1.92734pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) making 

Overfull \hbox (3.57817pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Bucinca, 

Overfull \hbox (3.45026pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) man+AI 

Overfull \hbox (1.0689pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dently"[]  

Overfull \hbox (2.52794pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) assisted 

Overfull \hbox (5.77692pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Decision- 

Overfull \hbox (1.92734pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) making 

Overfull \hbox (3.57817pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) Bucinca, 

Overfull \hbox (3.45026pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) man+AI 

Overfull \hbox (1.0689pt too wide) in paragraph at lines 21--21
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dently"[]  

LaTeX Warning: Citation 'rajpurkar2022ai' on page 1 undefined on input line 23.



LaTeX Warning: Citation 'goodell2021artificial' on page 1 undefined on input li
ne 23.


LaTeX Warning: Citation 'surden2019artificial' on page 1 undefined on input lin
e 23.


LaTeX Warning: Citation 'DBLP:conf/iclr/Saparov023' on page 1 undefined on inpu
t line 28.


LaTeX Warning: Citation 'DBLP:journals/tkdd/KaufmanRPS12' on page 1 undefined o
n input line 28.


LaTeX Warning: Citation 'DBLP:conf/nips/SolaimanD21' on page 1 undefined on inp
ut line 28.

[1.1{/var/lib/texmf/fonts/map/pdftex/updmap/pdftex.map}{/usr/share/texmf-dist/f
onts/enc/dvips/libertine/lbtn_25tcsq.enc}{/usr/share/texmf-dist/fonts/enc/dvips
/libertine/lbtn_76gpa5.enc}{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbt
n_naooyc.enc}{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_nh77jq.enc}{
/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_7grukw.enc}]

LaTeX Warning: Citation 'DBLP:conf/emnlp/CiosiciCLHFW21' on page 2 undefined on
 input line 51.


LaTeX Warning: Citation 'DBLP:conf/acl/ChenSFC0X23' on page 2 undefined on inpu
t line 51.


LaTeX Warning: Citation 'ferguson2020high' on page 2 undefined on input line 51
.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-1808-09123' on page 2 undefined
 on input line 53.


LaTeX Warning: Citation 'kempt2022m' on page 2 undefined on input line 53.


LaTeX Warning: Citation 'DBLP:conf/ijcai/RossHD17' on page 2 undefined on input
 line 53.


LaTeX Warning: Citation 'hildebrandt2013privacy' on page 2 undefined on input l
ine 56.


LaTeX Warning: Citation 'DBLP:conf/aaai/BansalW18' on page 2 undefined on input
 line 71.


LaTeX Warning: Citation 'DBLP:conf/hcomp/BansalNKLWH19' on page 2 undefined on 
input line 81.


Overfull \hbox (9.47112pt too wide) in paragraph at lines 81--81
\T1/LinuxLibertineT-TLF/m/n/6 (-20) bern[]etik[]es, 

Overfull \hbox (9.47112pt too wide) in paragraph at lines 81--81
\T1/LinuxLibertineT-TLF/m/n/6 (-20) bern[]etik[]es, 

LaTeX Warning: Citation 'dietvorst2018overcoming' on page 2 undefined on input 
line 81.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 2 undefined on input l
ine 82.

[2.2]

LaTeX Warning: Citation 'DBLP:journals/csur/YuZLHWJJ22' on page 3 undefined on 
input line 114.


LaTeX Warning: Citation '10.5555/3312046' on page 3 undefined on input line 114
.


LaTeX Warning: Citation 'DBLP:conf/ijcai/NobaniMM21' on page 3 undefined on inp
ut line 114.


Overfull \hbox (4.55762pt too wide) in paragraph at lines 168--169
 [][] 

Class acmart Warning: A possible image without description on input line 177.

[3.3]) (./paradigms.tex

Package caption Warning: \label without proper reference on input line 5.
See the caption package documentation for explanation.


LaTeX Warning: Reference `tbl:symbols' on page 4 undefined on input line 81.


LaTeX Warning: Citation 'Neykov2016' on page 4 undefined on input line 111.


LaTeX Warning: Citation 'Goodfellow2016' on page 4 undefined on input line 113.



LaTeX Warning: Citation 'Bartlett2006' on page 4 undefined on input line 113.


LaTeX Warning: Citation 'Lin2004' on page 4 undefined on input line 113.

[4.4{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_ki75ao.enc}{/usr/shar
e/texmf-dist/fonts/enc/dvips/libertine/lbtn_oexx6f.enc}] [5.5]

LaTeX Warning: Citation 'Lampert2016' on page 6 undefined on input line 130.


LaTeX Warning: Citation 'Kerrigan2021' on page 6 undefined on input line 132.

) (./human_oversight.tex

LaTeX Warning: Citation 'koulu2020proceduralizing' on page 6 undefined on input
 line 3.


LaTeX Warning: Citation 'quinonero2008dataset' on page 6 undefined on input lin
e 48.


Overfull \hbox (40.22641pt too wide) in paragraph at lines 48--54
[]\T1/LinuxLibertineT-TLF/m/it/10 (-20) Data shift. \T1/LinuxLibertineT-TLF/m/n
/10 (-20) Data shift is gen-er-ally in-tended as a change in the data dis-tri-b
u-tion [[]],
[6.6]

LaTeX Warning: Citation 'DBLP:journals/pacmhci/BucincaMG21' on page 7 undefined
 on input line 64.


LaTeX Warning: Citation 'parikh1994intuition' on page 7 undefined on input line
 67.


LaTeX Warning: Citation 'babuta2021machine' on page 7 undefined on input line 7
9.


LaTeX Warning: Citation 'malgieri2017right' on page 7 undefined on input line 7
9.


LaTeX Warning: Citation 'babuta2021machine' on page 7 undefined on input line 8
3.


LaTeX Warning: Citation 'ferguson2020high' on page 7 undefined on input line 83
.


LaTeX Warning: Citation 'gillespie2018custodians' on page 7 undefined on input 
line 83.


LaTeX Warning: Citation 'DBLP:conf/fat/RaghavanBKL20' on page 7 undefined on in
put line 84.


LaTeX Warning: Citation 'nahmias2021oversight' on page 7 undefined on input lin
e 87.


LaTeX Warning: Citation 'dietvorst2015algorithm' on page 7 undefined on input l
ine 108.


LaTeX Warning: Citation 'logg2019algorithm' on page 7 undefined on input line 1
08.


LaTeX Warning: Citation 'dietvorst2015algorithm' on page 7 undefined on input l
ine 110.


LaTeX Warning: Citation 'main2016cook' on page 7 undefined on input line 110.


Underfull \vbox (badness 1122) has occurred while \output is active [7.7]

LaTeX Warning: Citation 'alon2023human' on page 8 undefined on input line 124.


LaTeX Warning: Citation 'DBLP:journals/automatica/Bainbridge83' on page 8 undef
ined on input line 124.


LaTeX Warning: Citation 'ferguson2020high' on page 8 undefined on input line 12
4.


LaTeX Warning: Citation 'DBLP:conf/eaamo/Grgic-HlacaLWR22' on page 8 undefined 
on input line 125.


LaTeX Warning: Citation 'lee2018understanding' on page 8 undefined on input lin
e 125.


LaTeX Warning: Citation 'DBLP:conf/chi/0002HZ20' on page 8 undefined on input l
ine 126.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-1712-09124' on page 8 undefined
 on input line 126.


LaTeX Warning: Citation 'DBLP:conf/www/Grgic-HlacaRGW18' on page 8 undefined on
 input line 128.


Overfull \hbox (30.6207pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) place [[]] or fur-ther con-firm the stereo
-types [[],

Overfull \hbox (142.4989pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) agents tend to under-monitor when they per
-ceive affin-ity to-wards the mon-i-tor case at hand [[]],

Overfull \hbox (14.24838pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) or sim-ply when they deem their rea-son-in
g more ``hu-man'' than the ma-chine's [[]].

Overfull \hbox (38.19225pt too wide) in paragraph at lines 120--129
\T1/LinuxLibertineT-TLF/m/n/10 (-20) decision-making of the hu-man agents [[], 
[]].

LaTeX Warning: Citation 'englich2006playing' on page 8 undefined on input line 
132.


Overfull \hbox (2.2601pt too wide) in paragraph at lines 132--132
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 132--132
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

LaTeX Warning: Citation 'DBLP:journals/corr/abs-1812-03219' on page 8 undefined
 on input line 134.


LaTeX Warning: Citation 'albright2019if' on page 8 undefined on input line 134.



LaTeX Warning: Citation 'DBLP:journals/csur/GuidottiMRTGP19' on page 8 undefine
d on input line 140.


LaTeX Warning: Citation 'DBLP:conf/nips/LundbergL17' on page 8 undefined on inp
ut line 141.


LaTeX Warning: Citation 'DBLP:journals/expert/GuidottiMGPRT19' on page 8 undefi
ned on input line 141.


LaTeX Warning: Citation 'DBLP:conf/icml/KohL17' on page 8 undefined on input li
ne 141.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-2303-09297' on page 8 undefined
 on input line 141.


Overfull \hbox (80.86664pt too wide) in paragraph at lines 138--143
\T1/LinuxLibertineT-TLF/m/n/10 (-20) to fur-ther ex-plain the pre-dic-tions giv
en by a ma-chine. Ex-plain-able AI (XAI) [[]]
)

LaTeX Warning: Citation 'cortes2016l2r' on page 8 undefined on input line 273.

[8.8]

LaTeX Warning: Citation 'Chow1970' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'cortes2016l2r' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'Madras18' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'Mozannar20' on page 9 undefined on input line 279.


LaTeX Warning: Citation 'Madras18' on page 9 undefined on input line 285.

(./L2R.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (9.70471pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dovremmo 

Overfull \hbox (9.31847pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigma 

Overfull \hbox (8.02188pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) vazionalei[]  

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (9.70471pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) dovremmo 

Overfull \hbox (9.31847pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigma 

Overfull \hbox (8.02188pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) vazionalei[]  

LaTeX Warning: Citation 'Chow1970' on page 9 undefined on input line 3.


LaTeX Warning: Citation 'Chow1970' on page 9 undefined on input line 3.


LaTeX Warning: Citation 'ZhangSurv' on page 9 undefined on input line 6.


LaTeX Warning: Citation 'el_yaniv_foundation' on page 9 undefined on input line
 6.


LaTeX Warning: Citation 'HendrickxSurv' on page 9 undefined on input line 6.


LaTeX Warning: Citation 'HendrickxSurv' on page 9 undefined on input line 9.


LaTeX Warning: Citation 'HendrickxSurv' on page 9 undefined on input line 9.


LaTeX Warning: Citation 'ZhangSurv' on page 9 undefined on input line 9.


LaTeX Warning: Citation 'ZhangSurv' on page 9 undefined on input line 9.

[9.9]

LaTeX Warning: Citation 'GyorfiBayes' on page 10 undefined on input line 35.


LaTeX Warning: Citation 'outlier_survey_2004' on page 10 undefined on input lin
e 45.


LaTeX Warning: Citation 'anomaly_comprehensive_2020' on page 10 undefined on in
put line 45.


LaTeX Warning: Citation 'openset_surv' on page 10 undefined on input line 45.


Overfull \hbox (32.09886pt too wide) in paragraph at lines 45--46
\T1/LinuxLibertineT-TLF/m/it/10 (-20) tions\T1/LinuxLibertineT-TLF/m/n/10 (-20)
 . Most of the works in this par-tic-u-lar area frame the prob-lem as \T1/Linux
LibertineT-TLF/m/it/10 (-20) Out-lier de-tec-tion \T1/LinuxLibertineT-TLF/m/n/1
0 (-20) [[]]

LaTeX Warning: Citation 'Seo_Wallat_Graepel_Obermayer_2000' on page 10 undefine
d on input line 47.


LaTeX Warning: Citation 'Seo_Wallat_Graepel_Obermayer_2000' on page 10 undefine
d on input line 47.


LaTeX Warning: Citation 'Coles2001' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'Coles2001' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'Scheirer11' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'math11092171' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'ruddEVM' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'ruddEVM' on page 10 undefined on input line 47.


LaTeX Warning: Citation 'vignotto_extreme_2020' on page 10 undefined on input l
ine 47.


Overfull \hbox (74.74547pt too wide) in paragraph at lines 47--48
\T1/LinuxLibertineT-TLF/m/n/10 (-20) cesses as a test-ing point to un-der-stand
 whether to re-ject a data point or not [[]].
[10.10]

LaTeX Warning: Citation 'Coenen2020ProbabilityOD' on page 11 undefined on input
 line 49.


LaTeX Warning: Citation 'Coenen2020ProbabilityOD' on page 11 undefined on input
 line 49.


LaTeX Warning: Citation 'Landgrebe' on page 11 undefined on input line 49.


LaTeX Warning: Citation 'fewshotanom' on page 11 undefined on input line 49.


LaTeX Warning: Citation 'AsifNets' on page 11 undefined on input line 51.


LaTeX Warning: Citation 'AsifNets' on page 11 undefined on input line 51.


LaTeX Warning: Citation 'Dalitz2009RejectOA' on page 11 undefined on input line
 55.


LaTeX Warning: Citation 'Grandvalet2008' on page 11 undefined on input line 55.



LaTeX Warning: Citation 'Jnior2017NearestND' on page 11 undefined on input line
 55.


LaTeX Warning: Citation 'hansen_error_reject_1997' on page 11 undefined on inpu
t line 62.


LaTeX Warning: Citation 'el_yaniv_foundation' on page 11 undefined on input lin
e 62.


Overfull \hbox (3.87013pt too wide) in paragraph at lines 60--66
\T1/LinuxLibertineT-TLF/m/n/10 (-20) tion $\OML/nxlmi/m/it/10 f$\T1/LinuxLibert
ineT-TLF/m/n/10 (-20) , and $\OML/nxlmi/m/it/10 ^^\$ \T1/LinuxLibertineT-TLF/m/
n/10 (-20) is the thresh-old hy-per-pa-ram-e-ter [[], []].

LaTeX Warning: Citation 'battisti_democracy' on page 11 undefined on input line
 68.


LaTeX Warning: Citation 'sousa_map' on page 11 undefined on input line 68.


Overfull \hbox (20.76775pt too wide) in paragraph at lines 68--69
\T1/LinuxLibertineT-TLF/m/n/10 (-20) sider the class-wise vari-ance of these pr
e-dic-tions as in-di-ca-tion of un-cer-tainty [[],

LaTeX Warning: Citation 'destefano_shakespear' on page 11 undefined on input li
ne 69.


LaTeX Warning: Citation 'brinkrolf_lvq' on page 11 undefined on input line 69.


LaTeX Warning: Citation 'tortorella_svm' on page 11 undefined on input line 73.



LaTeX Warning: Citation 'tortorella_svm' on page 11 undefined on input line 73.



LaTeX Warning: Citation 'Johannes_interpretable_conf' on page 11 undefined on i
nput line 74.

[11.11]

LaTeX Warning: Citation 'capitaine_frelicot' on page 12 undefined on input line
 76.


LaTeX Warning: Citation 'ceccotti_vajda' on page 12 undefined on input line 76.



LaTeX Warning: Citation 'Fischer_multiple_tau' on page 12 undefined on input li
ne 77.


LaTeX Warning: Citation 'pillai' on page 12 undefined on input line 77.


LaTeX Warning: Citation 'Fischer_variance' on page 12 undefined on input line 7
7.


Overfull \hbox (2.31824pt too wide) in paragraph at lines 76--78
\T1/LinuxLibertineT-TLF/m/n/10 (-20) [[], []]. Mul-ti-ple lo-cal thresh-olds $\
OML/nxlmi/m/it/10 ^^\[]; [] ; ^^\[]$ \T1/LinuxLibertineT-TLF/m/n/10 (-20) [[]]

LaTeX Warning: Citation 'HendrickxSurv' on page 12 undefined on input line 79.


LaTeX Warning: Citation 'cortes2016l2r' on page 12 undefined on input line 79.


LaTeX Warning: Citation 'Bartlett2008' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'RamaswamyReject' on page 12 undefined on input line 80
.


LaTeX Warning: Citation 'pugnana2023' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'pugnana2023' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'Ziyin2019' on page 12 undefined on input line 80.


LaTeX Warning: Citation 'Grandvalet2008' on page 12 undefined on input line 81.



LaTeX Warning: Citation 'LIN2018' on page 12 undefined on input line 81.


LaTeX Warning: Citation 'Geifman2019SelectiveNetAD' on page 12 undefined on inp
ut line 81.


LaTeX Warning: Citation 'cortes2016l2r' on page 12 undefined on input line 86.


LaTeX Warning: Citation 'cortes2016l2r' on page 12 undefined on input line 86.

(/usr/share/texmf-dist/tex/latex/bbm-macros/ubbm.fd)

LaTeX Font Warning: Font shape `U/bbm/m/n' in size <5.5> not available
(Font)              size <5> substituted on input line 103.


LaTeX Warning: Citation 'Geifman2019SelectiveNetAD' on page 12 undefined on inp
ut line 109.

[12.12]

LaTeX Warning: Citation 'GeifmanNIPS17' on page 13 undefined on input line 111.



LaTeX Warning: Citation 'GeifmanNIPS17' on page 13 undefined on input line 111.



LaTeX Warning: Citation 'pmlr-v97-franc19a' on page 13 undefined on input line 
126.


LaTeX Warning: Citation 'JonesSKKL21' on page 13 undefined on input line 129.

) (./L2D.tex [13.13]

LaTeX Warning: Citation 'cortes2016l2r' on page 14 undefined on input line 75.


LaTeX Warning: Citation 'Madras18' on page 14 undefined on input line 77.


LaTeX Warning: Citation 'De2020Class' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Mozannar20' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Mozannar2023' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Okati2021' on page 14 undefined on input line 111.


LaTeX Warning: Citation 'Keswani2021' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Madras18' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Mozannar2023' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Martinez20' on page 14 undefined on input line 112.


LaTeX Warning: Citation 'Raghu2019TheAA' on page 14 undefined on input line 113
.


LaTeX Warning: Citation 'Verma2022Multi' on page 14 undefined on input line 128
.

[14.14]

LaTeX Warning: Citation 'Raghu2019TheAA' on page 15 undefined on input line 151
.


LaTeX Warning: Citation 'Raghu2019Med' on page 15 undefined on input line 152.


LaTeX Warning: Citation 'Bansal2021IsTM' on page 15 undefined on input line 156
.


LaTeX Warning: Citation 'Wilder2020' on page 15 undefined on input line 161.


LaTeX Warning: Citation 'Charusaie2022' on page 15 undefined on input line 164.



LaTeX Warning: Citation 'Charusaie2022' on page 15 undefined on input line 165.



LaTeX Warning: Citation 'Mozannar2023' on page 15 undefined on input line 173.


LaTeX Warning: Citation 'Mozannar2023' on page 15 undefined on input line 173.


Class acmart Warning: A possible image without description on input line 175.

[15.15]

LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 206.


LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 206.


LaTeX Warning: Citation 'Lin2004' on page 16 undefined on input line 210.


LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 211.


LaTeX Warning: Citation 'Charusaie2022' on page 16 undefined on input line 211.



LaTeX Warning: Citation 'Verma22' on page 16 undefined on input line 211.


LaTeX Warning: Citation 'Mozannar20' on page 16 undefined on input line 212.


LaTeX Warning: Citation 'Charusaie2022' on page 16 undefined on input line 217.


[16.16 <./media/joint_deferral_content_moderation.png>]

LaTeX Warning: Citation 'Liu2022' on page 17 undefined on input line 225.


LaTeX Warning: Citation 'Raman2021' on page 17 undefined on input line 226.


LaTeX Warning: Citation 'Dawid1982' on page 17 undefined on input line 229.


LaTeX Warning: Citation 'Verma22' on page 17 undefined on input line 229.


LaTeX Warning: Citation 'Verma22' on page 17 undefined on input line 229.


LaTeX Warning: Citation 'Bansal2021IsTM' on page 17 undefined on input line 234
.


LaTeX Warning: Citation 'Mozannar20' on page 17 undefined on input line 234.


LaTeX Warning: Citation 'Okati2021' on page 17 undefined on input line 234.


LaTeX Warning: Citation 'Raghu2019TheAA' on page 17 undefined on input line 234
.


LaTeX Warning: Citation 'Mozannar2023' on page 17 undefined on input line 237.


LaTeX Warning: Citation 'Madras18' on page 17 undefined on input line 249.


LaTeX Warning: Citation 'Mozannar20' on page 17 undefined on input line 249.


LaTeX Warning: Citation 'Pradier2021' on page 17 undefined on input line 250.


LaTeX Warning: Citation 'Madras18' on page 17 undefined on input line 250.

[17.17]

LaTeX Warning: Citation 'Wilder2020' on page 18 undefined on input line 255.


LaTeX Warning: Citation 'Mozannar2023' on page 18 undefined on input line 257.


LaTeX Warning: Citation 'Hemmer2022' on page 18 undefined on input line 285.


LaTeX Warning: Citation 'Verma2022Multi' on page 18 undefined on input line 287
.


LaTeX Warning: Citation 'Hemmer2022' on page 18 undefined on input line 289.


LaTeX Warning: Citation 'Gao2021' on page 18 undefined on input line 291.


LaTeX Warning: Citation 'Keswani2021' on page 18 undefined on input line 305.

[18.18]

LaTeX Warning: Citation 'Keswani2022' on page 19 undefined on input line 316.


LaTeX Warning: Citation 'Verma2022Multi' on page 19 undefined on input line 323
.


LaTeX Warning: Citation 'Shafer2008' on page 19 undefined on input line 323.


LaTeX Warning: Citation 'Angelopoulos2022' on page 19 undefined on input line 3
23.


LaTeX Warning: Citation 'Okati2021' on page 19 undefined on input line 329.


LaTeX Warning: Citation 'Mozannar2023' on page 19 undefined on input line 329.


LaTeX Warning: Citation 'De2020Class' on page 19 undefined on input line 331.


LaTeX Warning: Citation 'De2020Reg' on page 19 undefined on input line 331.


LaTeX Warning: Citation 'Leitao2022' on page 19 undefined on input line 342.


LaTeX Warning: Citation 'Hemmer2023' on page 19 undefined on input line 342.


LaTeX Warning: Citation 'Charusaie2022' on page 19 undefined on input line 344.



LaTeX Warning: Citation 'Cohn1994' on page 19 undefined on input line 344.

[19.19]

LaTeX Warning: Citation 'Hemmer2023' on page 20 undefined on input line 347.


LaTeX Warning: Citation 'Hemmer2023UserStudy' on page 20 undefined on input lin
e 359.


LaTeX Warning: Citation 'Papenmeier2023' on page 20 undefined on input line 362
.


LaTeX Warning: Citation 'Leitao2022' on page 20 undefined on input line 367.


LaTeX Warning: Citation 'Jones21' on page 20 undefined on input line 368.

[20.20]) (./human_interaction.tex

LaTeX Warning: Citation 'DBLP:journals/nn/VapnikV09' on page 21 undefined on in
put line 42.


LaTeX Warning: Citation 'DBLP:conf/kdd/BucilaCN06' on page 21 undefined on inpu
t line 42.


LaTeX Warning: Citation 'DBLP:journals/pieee/ZhuangQDXZZXH21' on page 21 undefi
ned on input line 42.


LaTeX Warning: Citation 'settles2009active' on page 21 undefined on input line 
42.


Overfull \hbox (43.57573pt too wide) in paragraph at lines 42--49
\T1/LinuxLibertineT-TLF/m/n/10 (-20) Trans-fer Learn-ing [[]], and Ac-tive Lear
n-ing [[]].

LaTeX Warning: Citation 'DBLP:journals/nn/VapnikV09' on page 21 undefined on in
put line 50.

[21.21]

LaTeX Warning: Citation 'DBLP:conf/kdd/BucilaCN06' on page 22 undefined on inpu
t line 70.


LaTeX Warning: Citation 'DBLP:journals/pieee/ZhuangQDXZZXH21' on page 22 undefi
ned on input line 93.


Overfull \hbox (149.376pt too wide) in paragraph at lines 93--97
\T1/LinuxLibertineT-TLF/m/n/10 (-20) tries to lever-age the knowl-edge of the T
eacher, and only then adapts it to the task at hand [[]].

LaTeX Warning: Citation 'settles2009active' on page 22 undefined on input line 
103.


LaTeX Warning: Citation 'settles2009active' on page 22 undefined on input line 
119.


LaTeX Warning: Citation 'DBLP:conf/nldb/MullerPBF22' on page 22 undefined on in
put line 119.


LaTeX Warning: Citation 'DBLP:journals/ml/CohnAL94' on page 22 undefined on inp
ut line 119.


LaTeX Warning: Citation 'DBLP:journals/ml/CohnAL94' on page 22 undefined on inp
ut line 120.

[22.22{/usr/share/texmf-dist/fonts/enc/dvips/libertine/lbtn_kijugd.enc}]
[23.23]
Overfull \hbox (2.2601pt too wide) in paragraph at lines 214--214
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 214--214
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (5.42758pt too wide) in paragraph at lines 216--216
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) Abbiamo 

Overfull \hbox (1.56297pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) roberto 

Overfull \hbox (8.2248pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigmi 

Overfull \hbox (5.7366pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) rezionale 

Overfull \hbox (1.65099pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) sezione 

Overfull \hbox (14.38783pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) l'importanza 

Overfull \hbox (4.70122pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) fragilita', 

Overfull \hbox (5.42758pt too wide) in paragraph at lines 216--216
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) Abbiamo 

Overfull \hbox (1.56297pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) roberto 

Overfull \hbox (8.2248pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) paradigmi 

Overfull \hbox (5.7366pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) rezionale 

Overfull \hbox (1.65099pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) sezione 

Overfull \hbox (14.38783pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) l'importanza 

Overfull \hbox (4.70122pt too wide) in paragraph at lines 216--216
\T1/LinuxLibertineT-TLF/m/n/6 (-20) fragilita', 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 217--217
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (5.5602pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) nell'altro 

Overfull \hbox (3.52669pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) munque 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 217--217
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (1.95529pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) gazioni, 

Overfull \hbox (5.5602pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) nell'altro 

Overfull \hbox (3.52669pt too wide) in paragraph at lines 217--217
\T1/LinuxLibertineT-TLF/m/n/6 (-20) munque 

LaTeX Warning: Marginpar on page 24 moved.


LaTeX Warning: Marginpar on page 24 moved.


Underfull \hbox (badness 10000) in paragraph at lines 219--222


Overfull \hbox (2.2601pt too wide) in paragraph at lines 244--244
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.4399pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) mento? 

Overfull \hbox (5.03302pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) potrebbe 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 244--244
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.4399pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) mento? 

Overfull \hbox (5.03302pt too wide) in paragraph at lines 244--244
\T1/LinuxLibertineT-TLF/m/n/6 (-20) potrebbe 

LaTeX Warning: Marginpar on page 24 moved.


Underfull \hbox (badness 10000) in paragraph at lines 259--269

[24.24]

Class acmart Warning: A possible image without description on input line 297.


LaTeX Warning: Citation 'DBLP:conf/cvpr/JohnsonHMFZG17' on page 25 undefined on
 input line 299.


LaTeX Warning: Citation 'DBLP:conf/iui/GuoDAMCK22' on page 25 undefined on inpu
t line 304.


LaTeX Warning: Citation 'DBLP:conf/pldi/EllisWNSMHCST21' on page 25 undefined o
n input line 312.

[25.25]

LaTeX Warning: Citation 'DBLP:conf/emnlp/KassnerTSC21' on page 26 undefined on 
input line 336.


LaTeX Warning: Citation 'DBLP:conf/nips/LewisPPPKGKLYR020' on page 26 undefined
 on input line 336.


LaTeX Warning: Citation 'DBLP:conf/ijcai/ClarkTR20' on page 26 undefined on inp
ut line 336.


Overfull \hbox (35.3791pt too wide) in paragraph at lines 336--343
\T1/LinuxLibertineT-TLF/m/n/10 (-20) builds on top of two other fam-i-lies, kno
wl-edge in-jec-tion mod-els [[]]

LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 380.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 380.


Class acmart Warning: A possible image without description on input line 382.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 384.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MishraTC22' on page 26 undefined on in
put line 390.


LaTeX Warning: Citation 'DBLP:conf/emnlp/BostromZCD21' on page 26 undefined on 
input line 392.


LaTeX Warning: Citation 'DBLP:conf/emnlp/MurtyMLR22' on page 26 undefined on in
put line 393.


LaTeX Warning: Citation 'DBLP:conf/nips/LewisPPPKGKLYR020' on page 26 undefined
 on input line 404.


LaTeX Warning: Citation 'DBLP:conf/aaai/HwangBBDSBC21' on page 26 undefined on 
input line 406.


LaTeX Warning: Citation 'DBLP:journals/cacm/VrandecicK14' on page 26 undefined 
on input line 406.


LaTeX Warning: Citation 'wang2017fvqa' on page 26 undefined on input line 431.

[26.26 <./media/clever.pdf>]

LaTeX Warning: Citation 'MalandriMMN23' on page 27 undefined on input line 457.



LaTeX Warning: Citation 'DBLP:journals/aim/AmershiCKK14' on page 27 undefined o
n input line 463.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 27 undefined on input 
line 463.

[27.27]
Overfull \hbox (2.2601pt too wide) in paragraph at lines 489--489
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.90285pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) lascerei 

Overfull \hbox (3.19742pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tostante 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 489--489
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (1.90285pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) lascerei 

Overfull \hbox (3.19742pt too wide) in paragraph at lines 489--489
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tostante 

LaTeX Warning: Citation 'DBLP:conf/ijcai/RossHD17' on page 28 undefined on inpu
t line 493.


LaTeX Warning: Citation 'teso2019toward' on page 28 undefined on input line 493
.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 28 undefined on input 
line 493.


LaTeX Warning: Citation 'DBLP:conf/aies/TesoK19' on page 28 undefined on input 
line 504.


LaTeX Warning: Citation 'DBLP:conf/kdd/WangKNSNCVV022' on page 28 undefined on 
input line 506.

[28.28 <./media/hydrant_only.png>]

LaTeX Warning: Citation 'Popordanoska2020' on page 29 undefined on input line 5
12.


LaTeX Warning: Citation 'DBLP:journals/corr/abs-2012-02898' on page 29 undefine
d on input line 514.


Overfull \hbox (40.68759pt too wide) in paragraph at lines 511--515
\T1/LinuxLibertineT-TLF/m/n/10 (-20) the cor-rec-tion is again an added com-po-
nent of the ma-chine ob-jec-tive [[]]. 

LaTeX Warning: Citation 'DBLP:journals/datamine/BontempelliGPT22' on page 29 un
defined on input line 517.

[29.29])
Overfull \hbox (9.70557pt too wide) in paragraph at lines 305--305
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) richiamare 

Overfull \hbox (9.70557pt too wide) in paragraph at lines 305--305
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) richiamare 

LaTeX Warning: Citation 'Sarkar2023' on page 30 undefined on input line 312.

[30.30] (./conclusions.tex)

LaTeX Warning: Empty bibliography on input line 338.

[31.31] (./appendices.tex

Class acmart Warning: \vspace should only be used to provide space above/below 
surrounding objects on input line 3.


Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (6.47256pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tosezione 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
[][][]\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (2.2601pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) FOSCA: 

Overfull \hbox (6.47256pt too wide) in paragraph at lines 3--3
\T1/LinuxLibertineT-TLF/m/n/6 (-20) tosezione 

LaTeX Warning: Citation 'Fisher1922' on page 32 undefined on input line 7.


LaTeX Warning: Citation 'Lin2004' on page 32 undefined on input line 8.


LaTeX Warning: Citation 'Bartlett2006' on page 32 undefined on input line 8.


LaTeX Warning: Citation 'Long2013' on page 32 undefined on input line 12.


LaTeX Warning: Citation 'Mozannar2023' on page 32 undefined on input line 14.


LaTeX Warning: Citation 'Verma22' on page 32 undefined on input line 14.


LaTeX Warning: Citation 'Lin2004' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Liu2007' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Tewari2007' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Zou2008' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Mozannar20' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Verma22' on page 32 undefined on input line 17.


LaTeX Warning: Citation 'Fisher1922' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Gerow1989' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Bartlett2006' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Lin2004' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Neykov2016' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Steinwart2007' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Tewari2007' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Bartlett2006' on page 32 undefined on input line 18.


LaTeX Warning: Citation 'Dawid1982' on page 32 undefined on input line 22.


LaTeX Warning: Citation 'Verma22' on page 32 undefined on input line 22.


LaTeX Warning: Citation 'Vaicenavicius2019' on page 32 undefined on input line 
22.


LaTeX Warning: Citation 'SilvaFilho2023' on page 32 undefined on input line 25.



LaTeX Warning: Citation 'Vaicenavicius2019' on page 32 undefined on input line 
29.


LaTeX Warning: Citation 'Kull2019' on page 32 undefined on input line 30.


LaTeX Warning: Citation 'SilvaFilho2023' on page 32 undefined on input line 30.


[32.32]

LaTeX Warning: Citation 'Verma2022Multi' on page 33 undefined on input line 32.



LaTeX Warning: Citation 'Verma22' on page 33 undefined on input line 32.


LaTeX Warning: Citation 'Verma22' on page 33 undefined on input line 40.


LaTeX Warning: Citation 'Verma2022Multi' on page 33 undefined on input line 40.



LaTeX Warning: Citation 'Long2013' on page 33 undefined on input line 46.


LaTeX Warning: Citation 'Long2013' on page 33 undefined on input line 46.


LaTeX Warning: Citation 'cortes2016l2r' on page 33 undefined on input line 47.


LaTeX Warning: Citation 'Mozannar20' on page 33 undefined on input line 47.


LaTeX Warning: Citation 'Mozannar2023' on page 33 undefined on input line 47.


LaTeX Warning: Citation 'cortes2016l2r' on page 33 undefined on input line 50.


LaTeX Warning: Citation 'Mozannar2023' on page 33 undefined on input line 50.


LaTeX Warning: Citation 'Mozannar20' on page 33 undefined on input line 50.


LaTeX Warning: Citation 'Mozannar2023' on page 33 undefined on input line 64.

[33.33] [34.34]
Overfull \hbox (10.90298pt too wide) in paragraph at lines 92--92
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Architecture| 

Overfull \hbox (5.88702pt too wide) in paragraph at lines 92--92
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Theoretical

Underfull \hbox (badness 10000) in paragraph at lines 92--92
\T1/LinuxLibertineT-TLF/m/n/10 (+20) guar-an-

Overfull \hbox (26.71838pt too wide) in paragraph at lines 92--92
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Constraints| 

LaTeX Warning: Citation 'Raghu2019TheAA' on page 35 undefined on input line 93.



Overfull \hbox (2.99666pt too wide) in paragraph at lines 93--93
[]|[]| 

Overfull \hbox (8.51001pt too wide) in paragraph at lines 93--93
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Budget| 

Underfull \hbox (badness 10000) in paragraph at lines 93--93
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Retinal

Underfull \hbox (badness 10000) in paragraph at lines 93--93
\T1/LinuxLibertineT-TLF/m/n/10 (+20) fun-dus

Underfull \hbox (badness 10000) in paragraph at lines 93--93
\T1/LinuxLibertineT-TLF/m/n/10 (+20) pho-

LaTeX Warning: Citation 'Wilder2020' on page 35 undefined on input line 94.


Underfull \hbox (badness 10000) in paragraph at lines 94--94
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Staged,

Underfull \hbox (badness 10000) in paragraph at lines 94--94
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 94--94
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy

Underfull \hbox (badness 10000) in paragraph at lines 94--94
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Zoo,

Underfull \hbox (badness 10000) in paragraph at lines 94--94
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Breast

LaTeX Warning: Citation 'Bansal2021IsTM' on page 35 undefined on input line 95.



Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) man

Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) credit,

Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) FICO,

Underfull \hbox (badness 10000) in paragraph at lines 95--95
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Com-pas,

LaTeX Warning: Citation 'Madras18' on page 35 undefined on input line 96.


Underfull \hbox (badness 10000) in paragraph at lines 96--96
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Joint

Overfull \hbox (14.13278pt too wide) in paragraph at lines 96--96
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Fairness,

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Cov-

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) er-

Underfull \hbox (badness 10000) in paragraph at lines 96--96
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Com-pas,

Underfull \hbox (badness 10000) in paragraph at lines 96--96
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Her-itage

LaTeX Warning: Citation 'Mozannar20' on page 35 undefined on input line 97.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 97--97
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) , CI-

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) FAR10H,

Underfull \hbox (badness 10000) in paragraph at lines 97--97
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CheX-

Overfull \hbox (22.41237pt too wide) in paragraph at lines 97--98
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/clinicalml/learn-

LaTeX Warning: Citation 'Verma22' on page 35 undefined on input line 98.


Overfull \hbox (8.51001pt too wide) in paragraph at lines 98--98
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Budget| 

Underfull \hbox (badness 10000) in paragraph at lines 98--98
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 10,

Overfull \hbox (6.44347pt too wide) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (-20) HAM10000,

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy-

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Zoo,

Underfull \hbox (badness 10000) in paragraph at lines 98--98
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate-

Overfull \hbox (5.80733pt too wide) in paragraph at lines 98--99
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/rajevv/OvA-

LaTeX Warning: Citation 'Charusaie2022' on page 35 undefined on input line 99.


Underfull \hbox (badness 10000) in paragraph at lines 99--99
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Lim-ited

Underfull \hbox (badness 10000) in paragraph at lines 99--99
\T1/LinuxLibertineT-TLF/m/n/10 (+20) hu-man

Underfull \hbox (badness 10000) in paragraph at lines 99--99
\T1/LinuxLibertineT-TLF/m/n/10 (+20) pre-dic-

Underfull \hbox (badness 10000) in paragraph at lines 99--99
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Overfull \hbox (87.11462pt too wide) in paragraph at lines 99--100
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/clinicalml/active_le
arn_to_defer| 

LaTeX Warning: Citation 'Liu2022' on page 35 undefined on input line 100.


Underfull \hbox (badness 10000) in paragraph at lines 100--100
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 100--100
\T1/LinuxLibertineT-TLF/m/n/10 (+20) MIMIC-

Underfull \hbox (badness 10000) in paragraph at lines 100--100
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Her-itage,

Underfull \hbox (badness 10000) in paragraph at lines 100--100
\T1/LinuxLibertineT-TLF/m/n/10 (+20) MIMIC-

Underfull \hbox (badness 10000) in paragraph at lines 100--101
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) https://github.com/liu-

Underfull \hbox (badness 10000) in paragraph at lines 100--101
\T1/LinuxLibertineT-TLF/m/n/10 (+20) res/Learning-to-Defer-with-

LaTeX Warning: Citation 'Raman2021' on page 35 undefined on input line 101.


Underfull \hbox (badness 10000) in paragraph at lines 101--101
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Synthetic

Underfull \hbox (badness 10000) in paragraph at lines 101--101
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

LaTeX Warning: Citation 'Pradier2021' on page 35 undefined on input line 102.


Underfull \hbox (badness 10000) in paragraph at lines 102--102
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Joint

Overfull \hbox (12.5326pt too wide) in paragraph at lines 102--102
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Sparsity

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) of

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) the

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) de-

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) fer-

Underfull \hbox (badness 10000) in paragraph at lines 102--102
\T1/LinuxLibertineT-TLF/m/n/10 (+20) ral

LaTeX Warning: Citation 'Mozannar2023' on page 35 undefined on input line 103.


Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Lim-ited

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) hu-man

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) pre-dic-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) tions,

Overfull \hbox (14.13278pt too wide) in paragraph at lines 103--103
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Fairness,

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Cov-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) er-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 10H,

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Speach,

Underfull \hbox (badness 10000) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Com-pas,

Overfull \hbox (5.06406pt too wide) in paragraph at lines 103--103
\T1/LinuxLibertineT-TLF/m/n/10 (-20) ChestXRay| 

Overfull \hbox (76.16968pt too wide) in paragraph at lines 103--104
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/clinicalml/human_ai_
deferral| 

LaTeX Warning: Citation 'Okati2021' on page 35 undefined on input line 104.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 104--104
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 104--104
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 104--104
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy-

Underfull \hbox (badness 10000) in paragraph at lines 104--105
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-11) https://github.com/Networks-

Underfull \hbox (badness 10000) in paragraph at lines 104--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Learning/differentiable-

LaTeX Warning: Citation 'De2020Class' on page 35 undefined on input line 105.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 105--105
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 105--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 105--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Stare,

Underfull \hbox (badness 10000) in paragraph at lines 105--105
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Mes-si-dor,

Underfull \hbox (badness 10000) in paragraph at lines 105--106
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-11) https://github.com/Networks-

Underfull \hbox (badness 10000) in paragraph at lines 105--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Learning/classification-

LaTeX Warning: Citation 'De2020Reg' on page 35 undefined on input line 106.


Overfull \hbox (17.98357pt too wide) in paragraph at lines 106--106
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Coverage| 

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Speech,

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Stare-H,

Underfull \hbox (badness 10000) in paragraph at lines 106--106
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Stare-D,

Underfull \hbox (badness 10000) in paragraph at lines 106--107
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-11) https://github.com/Networks-

Underfull \hbox (badness 10000) in paragraph at lines 106--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Learning/regression-under-

LaTeX Warning: Citation 'Hemmer2023' on page 35 undefined on input line 107.


Underfull \hbox (badness 10000) in paragraph at lines 107--107
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Limited

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hu-man

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Pre-dic-

Underfull \hbox (badness 10000) in paragraph at lines 107--107
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 100,

Overfull \hbox (5.06406pt too wide) in paragraph at lines 107--107
\T1/LinuxLibertineT-TLF/m/n/10 (-20) ChestXRay| 

Overfull \hbox (41.64806pt too wide) in paragraph at lines 107--108
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/ptrckhmmr/learning-

Underfull \hbox (badness 10000) in paragraph at lines 107--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) to-deferwith-limited-expert-

LaTeX Warning: Citation 'Hemmer2022' on page 35 undefined on input line 108.


Underfull \hbox (badness 10000) in paragraph at lines 108--108
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Speech,

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) CIFAR-

Underfull \hbox (badness 10000) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (+20) 100,

Overfull \hbox (5.06406pt too wide) in paragraph at lines 108--108
\T1/LinuxLibertineT-TLF/m/n/10 (-20) ChestXRay| 

Overfull \hbox (36.38547pt too wide) in paragraph at lines 108--109
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/ptrckhmmr/human-

LaTeX Warning: Citation 'Verma2022Multi' on page 35 undefined on input line 109
.


Underfull \hbox (badness 4846) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) of J,

Underfull \hbox (badness 10000) in paragraph at lines 109--109
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Overfull \hbox (6.44347pt too wide) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (-20) HAM10000,

Underfull \hbox (badness 10000) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Galaxy-

Underfull \hbox (badness 10000) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Zoo,

Underfull \hbox (badness 10000) in paragraph at lines 109--109
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate-

Overfull \hbox (29.51352pt too wide) in paragraph at lines 109--110
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/rajevv/Multi_L2D| 

LaTeX Warning: Citation 'Gao2021' on page 35 undefined on input line 110.


Underfull \hbox (badness 10000) in paragraph at lines 110--110
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Staged,

Underfull \hbox (badness 10000) in paragraph at lines 110--110
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 110--110
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Scene,

Underfull \hbox (badness 10000) in paragraph at lines 110--110
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Yeast,

Underfull \hbox (badness 10000) in paragraph at lines 110--110
\T1/LinuxLibertineT-TLF/m/n/10 (+20) MLC,

Overfull \hbox (16.05214pt too wide) in paragraph at lines 110--111
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/ruijiang81/hai-

LaTeX Warning: Citation 'Keswani2021' on page 35 undefined on input line 111.


Overfull \hbox (14.13278pt too wide) in paragraph at lines 111--111
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) Fairness,

Overfull \hbox (6.3736pt too wide) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (-20) Sparse

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) com-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) mit-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) tee,

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hu-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) man

Overfull \hbox (13.12315pt too wide) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (-20) dropout,

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hu-

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) man

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 111--111
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Hate

Overfull \hbox (48.74487pt too wide) in paragraph at lines 111--112
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/vijaykeswani/Deferra
l-

LaTeX Warning: Citation 'Keswani2022' on page 35 undefined on input line 112.


Underfull \hbox (badness 10000) in paragraph at lines 112--112
[]|\T1/LinuxLibertineT-TLF/m/n/10 (+20) Joint,

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Lim-ited

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) ground

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Real:

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Twit-ter

Underfull \hbox (badness 10000) in paragraph at lines 112--112
\T1/LinuxLibertineT-TLF/m/n/10 (+20) Eng-lish

Overfull \hbox (42.84532pt too wide) in paragraph at lines 112--113
[]|\T1/LinuxLibertineT-TLF/m/n/10 (-20) https://github.com/vijaykeswani/Online-

[35.35] [36.36] [37.37] [38.38]
(/usr/share/texmf-dist/tex/generic/stringenc/se-pdfdoc.def)
(/usr/share/texmf-dist/tex/generic/stringenc/se-utf8.def) [39.39])

LaTeX Warning: Empty bibliography on input line 348.


Class acmart Warning: Some images may lack descriptions.

(./main.aux (./appendices.aux))

LaTeX Font Warning: Size substitutions with differences
(Font)              up to 0.5pt have occurred.


LaTeX Warning: There were undefined references.


Package biblatex Warning: Please (re)run Biber on the file:
(biblatex)                main
(biblatex)                and rerun LaTeX afterwards.

 )
(see the transcript file for additional information) </home/aslan/.texlive/texm
f-var/fonts/pk/ljfour/public/bbm/bbm10.600pk></usr/share/texmf-dist/fonts/type1
/public/newtx/LibertineMathMI.pfb></usr/share/texmf-dist/fonts/type1/public/new
tx/LibertineMathMI5.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/Liberti
neMathMI7.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/LibertineMathRM.p
fb></usr/share/texmf-dist/fonts/type1/public/libertine/LinBiolinumT.pfb></usr/s
hare/texmf-dist/fonts/type1/public/libertine/LinBiolinumTB.pfb></usr/share/texm
f-dist/fonts/type1/public/libertine/LinBiolinumTI.pfb></usr/share/texmf-dist/fo
nts/type1/public/libertine/LinLibertineT.pfb></usr/share/texmf-dist/fonts/type1
/public/libertine/LinLibertineTB.pfb></usr/share/texmf-dist/fonts/type1/public/
libertine/LinLibertineTBI.pfb></usr/share/texmf-dist/fonts/type1/public/liberti
ne/LinLibertineTI.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/NewTXMI.p
fb></usr/share/texmf-dist/fonts/type1/public/newtx/NewTXMI7.pfb></usr/share/tex
mf-dist/fonts/type1/public/newtx/stxscr.pfb></usr/share/texmf-dist/fonts/type1/
public/newtx/txexas.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/txexs.p
fb></usr/share/texmf-dist/fonts/type1/public/newtx/txmiaX.pfb></usr/share/texmf
-dist/fonts/type1/public/txfonts/txsyb.pfb></usr/share/texmf-dist/fonts/type1/p
ublic/txfonts/txsyc.pfb></usr/share/texmf-dist/fonts/type1/public/newtx/txsys.p
fb>
Output written on main.pdf (39 pages, 2846366 bytes).
Transcript written on main.log.
This is BibTeX, Version 0.99d (TeX Live 2023/Arch Linux)
The top-level auxiliary file: main.aux
I found no \citation commands---while reading file main.aux
I found no \bibdata command---while reading file main.aux
I found no \bibstyle command---while reading file main.aux
(There were 3 error messages)

